Unsupervised Point Cloud Pre-Training via Occlusion Completion

We describe a simple pre-training approach for point clouds. It works in three steps: 1. Mask all points occluded in a camera view; 2. Learn an encoder-decoder model to reconstruct the occluded points; 3. Use the encoder weights as initialisation for downstream point cloud tasks. We find that even when we construct a single pre-training dataset (from ModelNet40), this pre-training method improves accuracy across different datasets and encoders, on a wide range of downstream tasks. Specifically, we show that our method outperforms previous pre-training methods in object classification, and both part-based and semantic segmentation tasks. We study the pre-trained features and find that they lead to wide downstream minima, have high transformation invariance, and have activations that are highly correlated with part labels. Code and data are available at: https://github.com/hansen7/OcCo

==> OcCo ICCV 2021/sections/abstract.tex <==
%There has recently been a flurry of exciting advances in deep learning models on point clouds. However, these advances have been hampered by the difficulty of creating labelled point cloud datasets: sparse point clouds often have unclear label identities for certain points, while dense point clouds are time-consuming to annotate. We describe a %%%% HERE
We propose a surprisingly simple pre-training approach for point clouds. Inspired by mask-based pre-training in the natural language processing community, it works in three steps: 1. Mask all points that are occluded in different camera views; 2. Learn an encoder-decoder model to reconstruct the occluded points; 3. Use the encoder weights  as initialization for any downstream task. Surprisingly, we find that even when we construct a single pre-training dataset (from ModelNet40), the pre-trained encoder improves accuracy on a wide range of downstream tasks, across different datasets and encoder models. Specifically, we show that this method is competitive with recent work in the few-shot learning setting. At the same time it improves final generalization accuracy in object classification, part and semantic segmentation tasks. To better understand this approach, we investigate the pre-trained weights using various probe tests and visualizations. Code is available at https://anonymous.

%It then optimizes a completion model that learns how to reconstruct the occluded points, given the partial point cloud. In this way, our method learns a pre-trained representation that can identify the visual constraints inherently embedded in real-world point clouds. 
%We call our method \emph{Occlusion Completion} (OcCo). 
%learns representations that improve the semantic understandings as well as generalization on downstream tasks over prior methods, %that
%transfer to different datasets, %that
%reduce training time and improve label efficiency.
% sample efficiency. 
% Our code and dataset are available at \href{https://github.com/hansen7/OcCo}{{\color{blue}https://github.com/hansen7/OcCo}}.


==> OcCo ICCV 2021/sections/discussion.tex <==
%!TEX root = ../main.tex
In this work, we have demonstrated that why and how the Occlusion Completion (OcCo) learns the representations on point clouds that are more transformation invariant, more accurate in few-shot learning, and in various classification and segmentation fine tuning tasks, compared to prior work.
% generalizable representations for a variety of point cloud learning tasks, while increasing labelled sample efficiency and model convergence speed. %Further, these representations accelerate training fully-supervised learning. 
% \todo{to reduce a few in the future works.}
% There are a few exciting directions that we would like to explore in future. 
% First, we believe this method would be useful as a data-augmentation technique during training to improve robustness, similar to input dropout in the 2D case \citet{bouthillier2015dropout}. 
%The idea is that if a model is still good at say, classification, from partial point clouds, it will likely generalize better to unseen point clouds. 
% Second, 
In future, 
it would be interesting to design a completion model that is explicitly aware the view-point of the occlusion. 
% that it is completing an occluded view-point. 
A model like this would likely converge even quicker, and require fewer parameters, as this knowledge could act as a stronger inductive bias during learning. 
%Third, we believe there are a host of other 3D computer graphics concepts that could be leveraged to learn improved representations %generalizable and computationally efficient representations 
%for point cloud data.  %Specifically, a model that tries to predict how polygon meshes of 3D point clouds cast shadows would likely have a generic understanding of the 3D object behind the point cloud. 
%Similarly, a model that learns how to distinguish incoming versus emitted spectral radiance of a 3D surface via a deep parameterization of the rendering equation would likely produce a representation that improves classification and segmentation. 
In general, we advocate for structuring deep models using graphical constraints as an inductive bias to improve learning.

% \paragraph{Acknowledgements}
% Hanchen would acknowledge the support from Cathy Xu Fellowship, Cambridge Trust Scholarship and CAPA Award, as well as Cambridge Engineering technician team.

==> OcCo ICCV 2021/sections/experiments.tex <==
\newcommand{\qi}[1]{\textcolor{green}{\bf [Qi: #1]}}
\qi{1. Change standard deviation to standard error. 2. We color \textcolor{blue}{blue} the best results for each encoder and \textbf{bold} in black the overall best result for each dataset. 3. tidy the appendix section. }
%!TEX root = ../main.tex
% \begin{figure}[t!]
%     \centering
%     \vspace{-7ex}
%     \includegraphics[width=.9\linewidth]{resources/occlusion_steps.pdf}
%     \vspace{-1ex}
%     \caption{Overview of the procedure to generate occluded point clouds. See text for details.}
%     \label{fig:occlusion_steps}
%     \vspace{-2ex}
% \end{figure}

% We evaluate \abbrev on various downstream tasks, models, and datasets. 
%In Section \ref{sec:pretrain_settings}, we present the datasets and pre-training settings. We then show results on object classification tasks in Section \ref{sec:classification}, and semantic segmentation in Section \ref{sec:scene_seg}. In Section \ref{sec:efficiency}, we demonstrate that in cases where labelled data is particularly sparse, our method boosts accuracy. Related to this, models with \abbrev initialization converge faster to better test accuracies than randomly initialized models, which we show in Section~\ref{subsec:train_convergence}. Finally, we present further results on the sensitivity of our model to hyperparameter choices in the appendix. 
% All experiments are conducted on a 8-core NVIDIA GTX 1080 cluster and a 10-core NVIDIA RTX 6000 cluster.
%\abbrev improves sample efficiency. More experiments are presented in the appendix.

%our method improves representation learning with faster convergence speed and better scores. Then we investigate how our method perform when providing less training data.
%and finally we evaluate how sensitive our model is to the settings of \abbrev pre-training. 
% We then evaluate the transferability of the learned representations, and how they affect training convergence. 
% Finally, we demonstrate our method improves learning with less training labels, 

%In the appendix, we also include how we choose which weights from the \abbrev pre-training to be restored for the downstream tasks, and the difference between our constructed self-occluded point cloud data based on ModelNet40 and the other one based on ShapeNet which is used in the previous work\cite{yuan2018pcn,Tchapmi_2019_CVPR,abs-2004-03327} on point cloud completion.

In this section, we first present the details of OcCo pre-training (Section \ref{sec:pretrain_settings}), and fine-tuning (Section \ref{fine_tuning_details}). The results of few-shot learning, object classification, part segmentation and semantic segmentation are shown in Section \ref{fine_tuning_results}.


\subsection{OcCo Pre-Training Details \label{sec:pretrain_settings}}

% We now describe the datasets, models, and tasks we use for evaluation.
% of \abbrev.

%\textit{\abbrev pre-training details}: %For the occlusion completion pretraining tasks, we use PCN and PointNet to encode the global features of the occluded point cloud, and the two-stage decoder to generate the coarse and fine completed point cloud. Each object is normalised into unit sphere and repeatedly sampled or downsampled into 1024 points, the number of points in the coarse and detailed outputs are 1024 and 16384 respectively.
% some of the examples are visualised in Figure.~\ref{fig:dataoverview}.

% \todo{Add More, as in the Commented Paragraphs. Maybe put the architecture details into appendix and refer to it?}

% \subsection{Technical Details}
% We first describe how we generate the occluded point clouds. The intrinsics of the camera (in eq.~\ref{eq:camera_transform}) are set to $f=1000, \gamma=0, \omega=1600, h=1200$. For each polygon mesh, we normalise it into unit sphere and choose three angles uniformly from $[0, 2\pi]$ as the value for yaw, pitch, roll: $r_{\{1...9\}}$. The object is centered at the origin of the world frame with zero translations: $t_{\{1,2,3\}}$. Then we use z-buffering to render it into a depth image. The self-occluded point clouds are generated via back-projecting the depth images based on eq.~\ref{eq:world_transform}.
% We choose ModelNet40 as it has a richer class of objects compared to other datasets. 
% Specifically, 
% We sample 10 sets of yaw, pitch and roll uniformly from $[0, 2\pi]$ which yield $\{r_{1}, \ldots, r_9\}$,
% via the standard Euler angle transformation, 
% and set zero translation $t_{\{1,2,3\}}\!=\!0$. 
\textbf{Dataset}: For all experiments, we use ModelNet40~\citep{wu20153d} as the pre-training dataset, a challenging transfer learning setting, as ModelNet40 and fine-tuning datasets may not come from the same domain. ModelNet40 includes 12,311 synthesized objects from 40 categories, divided into 9,843/2,468 objects for training and testing, respectively. We construct a pre-training dataset using the training objects. We generate occluded point clouds with camera intrinsic parameters $\{f=1000, \gamma=0, \omega=1600, h=1200$\}, 10 randomly selected viewpoints and zero translation. Figure~\ref{fig:dataoverview} shows examples of occluded point clouds. 
% Note that these are qualitatively similar to point clouds in datasets where points are collected via 3D imaging devices such as handheld scanners \citep{dai2017scannet,armeni20163d}
% % (ScanNet: \citet{dai2017scannet}, S3DIS, \citet{armeni20163d}) 
% and lidar \citep{KITTI}. 
% (KITTI, \citet{KITTI}). 

% encoders, similar to prior completion models~\citep{Tchapmi_2019_CVPR,WangAL20,WenLHL20}

\textbf{Architecture}: Our pre-training model, a completion model $c(\cdot)$, follows the ``encoder-decoder'' architecture. To validate the generality of our pre-training objective, we choose three different encoders including PointNet~\citep{qi2017pointnet}, PCN~\citep{yuan2018pcn} and DGCNN~\citep{wang2019dynamic}. These encoders encode an occluded point cloud into a 1024-dimensional vector. For decoder, we adapt the folding-based decoder from \citet{yuan2018pcn} to complete an occluded point cloud in two steps. The decoder first output a coarse shape, $\hat{\mathcal{P}}_{coarse}$, with 1024 points then warps a 2D grid around each point in $\hat{\mathcal{P}}_{coarse}$ in order to get a fine shape, $\hat{\mathcal{P}}_{fine}$, which consist of 16384 points. We use Chamfer Distance (CD) as the closeness measure of two point sets:
\begin{gather}
\begin{split}
    \mathrm{CD}(\hat{\mathcal{P}}, \mathcal{P}) = &\frac{1}{|\hat{\mathcal{P}}|}\sum_{\hat{x}\in \hat{\mathcal{P}}}\min_{x\in \mathcal{P}}||\hat{x}-x||_2 \\+ &\frac{1}{|\mathcal{P}|}\sum_{x\in \mathcal{P}}\min_{\hat{x}\in \hat{\mathcal{P}}}||x-\hat{x}||_2.
\end{split}
\end{gather}
The total loss of the completion task is a linear combination of the two Chamfer Distances:
\begin{gather}\label{eq:completion_loss}
    l = \mathrm{CD}(\hat{\mathcal{P}}_{coarse}, \mathcal{P}_{coarse}) + \alpha * \mathrm{CD}(\hat{\mathcal{P}}_{fine}, \mathcal{P}_{fine}),
\end{gather}

% It first generates a sparse set of points to match the overall geometry of the point cloud. Then it generates dense points around the sparse points to approximate a smooth surface. 
% , as we find it performs just as well as the Earth Mover's Distance (EMD), which is slower and must be approximated to run practically~\citet{bertsekas1985distributed}. 
% For further optimization details and a hyperparameter sensitivity study, see the Appendix.
% \paragraph{\abbrev pre-training.}

\textbf{Hyperparameters}: We use Adam~\citep{KingmaB14} as the optimizer. The learning rate is set to 1e-4 initially, and is decayed by 0.7 every 10 epochs. We pre-train the models for 50 epochs. The batch size is 32 and the momentum of batch normalisation is 0.9. The coefficient $\alpha$ in~\eqref{eq:completion_loss} is first set as 0.1 for the first 10000 training steps, then increases to 0.1 and 0.5 at the 20000th and 50000th training steps, respectively. The $\alpha$ is fixed as 1.0 after 50000 training steps. 

\begin{table*}[h!]
\small
\centering
% \vspace{-1ex}
\caption{Comparison between \abbrev, Jigsaw and Rand initialization on 3D object recognition benchmarks.
% , based on PointNet, PCN and DGCNN. 
% Here `*' marks the reported scores from the original literature \citep{qi2017pointnet,wang2019dynamic,ScanObjectNN,sauder2019self} (we additionally confirm these scores are reproducible). 
After confirming the scores from \citep{qi2017pointnet,wang2019dynamic,ScanObjectNN,sauder2019self} are reproducible, we reported the mean and standard deviation over three runs.} % `**' marks our reproduced result which is quite lower than reported in \cite{ScanObjectNN} with the same protocols}
%For the benchmark datasets, the first three, `ShapeNet10', `ModelNet10' and `ModelNet40' are fully synthesized 3D objects based on CAD models, while `ScanNet10' contained the same class as `ShapeNet10' and `ModelNet10' but with occlusion. `ShapeNet Par' and `ModelNet Par' are the data we used for \abbrev tasks, consist of synthesized occluded point clouds, 
% `ScanObjectNN' includes real-world point cloud, which are segmented from entire indoor scans which are occluded, sometime with background noise (bn), we list all the test results on the variations of `ScanObjectNN' in the appendix.
% \vspace{-1ex}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{Dataset} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
% ShapeNet10 & 94.9 & 95.3 & \textcolor{blue}{95.5} & 95.1 & 95.2 & \textcolor{blue}{95.4} & 95.8 & 96.0 & \textbf{96.6} \\\hline
MN40& 89.2$\pm$0.2 & 89.6$\pm$0.2 & \textcolor{blue}{90.1$\pm$0.2} & 89.3$\pm$0.2 & 89.6$\pm$0.3 & \textcolor{blue}{90.3$\pm$0.3} & 92.5$\pm$0.7 & 92.3$\pm$0.5 & \textbf{93.0$\pm$0.3} \\\hline
% ShapeNet Oc & 94.6 & 94.6 & \textcolor{blue}{95.0} & 94.9 & \textbf{95.1} & \textbf{95.1} & 94.5 & 94.4 & \textbf{95.1} \\\hline
% ModelNet Oc & 85.3$\pm$0.2 & 85.5 & \textcolor{blue}{85.6} & 84.6 & \textcolor{blue}{85.1} & \textcolor{blue}{85.1} & 88.7 & 88.7 & \textbf{89.1} \\\hline
ScN10& 76.9$\pm$0.3 & 77.2$\pm$0.3 & \textcolor{blue}{78.0$\pm$0.3} & 77.0$\pm$0.5 & 77.9$\pm$0.5 & \textcolor{blue}{78.2$\pm$0.5} & 76.1$\pm$1.2 & 77.8$\pm$0.9 & \textbf{78.5$\pm$0.5}  \\\hline
SO15 & 73.5$\pm$0.9 & 76.5$\pm$0.7 & \textcolor{blue}{80.0$\pm$0.3} & 78.3$\pm$0.5 & 78.2$\pm$0.2 & \textcolor{blue}{80.4$\pm$0.3} & 82.4$\pm$0.7 & 82.7$\pm$1.4 & \textbf{83.9$\pm$0.7} \\
% ScanObjectNN (OBJ\_ONLY)\cite{ScanObjectNN}& 79.2* & 79.9 & 79.3 & 79.5 & 79.7** & 84.0\\
\toprule
\end{tabular}
\label{tab:classification}
% \vspace{-3ex}
\end{table*}

\subsection{Fine-Tuning Details \label{fine_tuning_details}}
% while Unseen samples are then queried from 
% for testing

% \qi{The contents of this section are a bit cluttered. We can first introduce the four tasks and then introduce the fine-tuning hyperparameters}

\paragraph{Few-shot learning.} Few-shot learning aims to build accurate models with very limited training data, and a common setting is called ``$K$-way $N$-shot''. During training, $K$ classes are randomly selected, and each class contains $N$ samples. The trained model are then evaluated on the objects from the test split. In our experiments, we use ModelNet40 and Syndey10~\citep{de2013unsupervised} for the ``$K$-way $N$-shot'' classification. We use the same setting and train/test split as cTree \citep{sharma2020self}. Each object is represented with 100 points. We use the same training configurations as in the object classification tasks.


%We use the same training settings as used in the next paragraph. 
% The training settings are identical to the ones used in the classification.
% We use the same data and train/test split as \citep{sharma2020self}, the training settings are identical to previous.
% We use the same training settings as our classification experiments, which are identical to the original literature.

\paragraph{Object classification.}
Given an object represented by a set of points, object classification is to predict which class this object belongs to.
We use three 3D object recognition benchmarks: ModelNet40~\cite{wu20153d}, ScanNet10~\citep{pointdan} and ScanObjectNN~\citep{ScanObjectNN}. We summarise the dataset statistics in table~\ref{tab:classification_benchmark}, where the later two are more challenging since they contain the occluded objects from the real indoor scans.
We use the same training settings as the original works. Concretely, for PCN and PointNet, we use the Adam optimizer with an initial learning rate 1e-3, decayed by 0.7 every 20 epochs to a minimum value of 1e-5. For DGCNN, we use the SGD optimizer with a momentum of 0.9 and a weight decay of 1e-4. The learning rate starts from 0.1 and then reduces using cosine annealing~\cite{LoshchilovH17} with a minimum value of 1e-3. We use dropout~\cite{dropout} in the fully connected layers before the softmax output layer. The dropout rate of PointNet and PCN is set to 0.7, and is 0.5 for DGCNN. For all three models, we train them for 200 epochs with a batch size of 32. We report the test results based on three runs in table~\ref{tab:classification}.

\begin{table}[H]
\centering
\small
\vspace{-2ex}
\caption{Statistics of classification datasets}
\begin{tabular}{l|c|c|c|c}
\bottomrule 
Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
MN40& synthesized & 40 & 9,843 & 2,468 \\\hline
% ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
SN10 & real scanned & 10 & 6,110 & 1,769 \\\hline
SO15 & real scanned & 15 & 2,304 & 576 \\
\toprule
\end{tabular}
\label{tab:cls_data}
\vspace{-3ex}
\end{table}

% : ModelNet40, ShapeNet10, ScanNet10, ShapeNet Occluded, ModelNet Occluded and ScanObjectNN (OBJ\_BG). 
% For PointNet and DGCNN baselines, we use the same training settings as the original literature, we adapt the output layers as well as the training setting for PCN based on those of PointNet (in appendix).
% , just as in~\citeps{qi2017pointnet}. 
% : ShapeNet~\cite{chang2015shapenet}, ModelNet40~\cite{wu20153d} and ScanNet10~\cite{pointdan}.
% ShapeNet has more than 3 million CAD models, of which 220,000 models are labeled into 3,135 object categories, making it one of the largest 3D object classification datasets.
% ADD MODELNET
%ShapeNet10 and ScanNet10 are first introduced for domain adaptation~\cite{pointdan}.
% does the below sound okay? this way we don't say we introduce it
% it's a bit confusing to say it was introduced by PCN as they would have to know our model to use our technique, I realize our technique is based on PCN, but I just think it's clearer to say 'we use our occlusion technique' to create both datasets
% hmmm, I see. maybe we can just say in the appendix that we need to improve the quality of that data before using it for pre-training?
% good point
% could we submit the main paper then?
% thanks!
% ohoh, I just want to be consistent with the appendix since the model pre-trained on shapenet occluded mostly performance even worse than random insitilaised ones, that is probably because of the quality of pre-trained data, which is not our responsibility
% okay, this is not the place where the reviewer cares about..
% yead, on it
% ShapeNet10 is sampled from the synthesized dataset ShapeNet~\cite{chang2015shapenet} with 17,378 training examples and 2,492 testing examples. ScanNet10 is derived from scanned and reconstructed real-world indoor scenes~\cite{dai2017scannet} with 6,110  training examples and 1,769 testing examples. We also evaluate on ShapeNet Occluded and ModelNet Occluded, where we use the occlusion mapping described in Section~\ref{subsec:occ} to create occluded point clouds. These datasets are used to evaluate the models on a more challenging scenario where point clouds are partially observable. ModelNet Oc contains 98,430 training CAD models and 24,680 testing models, while ShapeNet Oc consists of 231,792 training examples and 800 testing examples. We also use a real-world scanned indoor scene dataset, ScanObjectNN (OBJ\_BG)~\cite{ScanObjectNN}, which contains 15 categories, 2,304 training objects and 576 testing objects. All point clouds are sub-sampled to 1024 points, just as in~\citet{qi2017pointnet}.
% \begin{table}[H]
% \centering
% \small
% \vspace{-2ex}
% \caption{Statistics of classification datasets}
% \vspace{-2ex}
% \begin{tabular}{l|c|c|c|c}
% \bottomrule 
% Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% % ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
% (MN40) ModelNet40~\citep{wu20153d} & synthesized & 40 & 9,843 & 2,468 \\\hline
% % ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% % ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
% (SN10) ScanNet10~\citep{dai2017scannet} & real scanned & 10 & 6,110 & 1,769 \\\hline
% (SO15) ScanObjectNN ~\citep{ScanObjectNN} & real scanned & 15 & 2,304 & 576 \\
% \toprule
% \end{tabular}
% \label{tab:cls_data}
% \vspace{-3ex}
% \end{table}

\paragraph{Part segmentation.} 
Part segmentation is a challenging fine-grained 3D recognition task. Given a 3D scan, the task is to predict part category label (e.g., chair leg, cup handle) of each point.
We use the ShapeNetPart~\citep{armeni20163d} benchmark for this task, which contains 16,881 objects from 16 categories, and has 50 parts in total.
Each object is represented with 2048 points. We use the same training settings as the original works, for PCN and PointNet, we use the Adam optimizer with an initial learning rate 1e-3, decayed by 0.5 every 20 epochs to a minimum value of 1e-5. For DGCNN, we use the SGD optimizer with a momentum of 0.9 and a weight decay of 1e-4. The learning rate starts from 0.1 and then reduces using cosine annealing~\cite{LoshchilovH17} with a minimum value of 1e-3. For all three models, we train them for 250 epochs with a batch size of 16. We use the same test procedures (majority votes) as the original works, and report the results based on three runs in table~\ref{tab:partseg_result}.


\paragraph{Semantic segmentation.} 
Similar to part segmentation, the point labels in semantic segmentation instead become semantic object classes of an indoor/outdoor scene. We use the S3DIS benchmark~\citep{armeni20163d} for semantic indoor scene segmentation. It contains 3D scans collected via Matterport scanners in 6 different places, encompassing 271 rooms. Each point, described by a 9-dimensional vector (including coordinates, RGB values and normalised location), is labeled as one of 13 semantic categories (e.g. chair, table and floor). We use the same preprocessing procedures and training settings as the original work. 
We also fine tuned and show the effectiveness of our pre-training on a recent urban-scale outdoor point cloud scans~\cite{hu2020towards}. We reported these results in the appendix.

\begin{table}[h!]\small
\centering
% \vspace{-2ex}
\setlength{\tabcolsep}{2pt}
\caption{Few-shot classification results. We report mean and std over 10 runs. We bold the the cell with the largest mean.
% We also bold the cell where its mean + std $>=$ the largest mean.
\label{exp:few_shot_classification} }
\begin{tabular}{l|cccc}
\bottomrule \multicolumn{1}{c|}{\multirow{2}{*}{Baseline}} 
& \multicolumn{2}{c}{5-way} & \multicolumn{2}{c}{10-way} \\ \cline{2-5}
& 10-shot & 20-shot & 10-shot & 20-shot \\ \toprule \bottomrule
3D-GAN & 55.8$\pm$10.7 & 65.8$\pm$9.9 &40.3$\pm$6.5 &48.4$\pm$5.6\\
FoldingNet & 33.4 $\pm$13.1 & 35.8$\pm$18.2 & 18.6$\pm$6.5 & 15.4$\pm$6.8 \\
Latent-GAN & 41.6$\pm$16.9 & 46.2$\pm$19.7 & 32.9$\pm$9.2 & 25.5$\pm$9.9\\
PointCapsNet & 42.3$\pm$17.4 &53.0$\pm$18.7 &38.0$\pm$14.3 & 27.2$\pm$14.9\\
PointNet++ & 38.5$\pm$16.0 & 42.4$\pm$14.2 & 23.1$\pm$7.0 & 18.8$\pm$5.4 \\
PointCNN & {65.4$\pm$8.9} & {68.6$\pm$7.0} & {46.6$\pm$4.8} & {50.0$\pm$7.2} \\
\toprule \bottomrule
PointNet, Rand & 52.0$\pm$12.2 & 57.8$\pm$15.5 & 46.6$\pm$13.5 & 35.2$\pm$15.3 \\
PointNet, cTree & 63.2$\pm$10.7 & 68.9$\pm$9.4 & 49.2$\pm$6.1 & 50.1$\pm$5.0 \\
PointNet, OcCo & \textbf{89.7$\pm$6.1} & \textbf{92.4$\pm$4.9} & \textbf{83.9$\pm$5.6} & \textbf{89.7$\pm$4.6} \\\hline
DGCNN, Rand & 31.6 $\pm$9.0 & 40.8$\pm$14.6 &19.9$\pm$6.5 & 16.9$\pm$4.8\\
DGCNN, cTree & 60.0$\pm$8.9 & 65.7$\pm$8.4 & 48.5$\pm$5.6 & 53.0$\pm$4.1\\
DGCNN, OcCo & \textbf{90.6$\pm$2.8} & \textbf{92.5$\pm$6.0} & \textbf{82.9$\pm$4.1} & \textbf{86.5$\pm$7.1}\\
\toprule
\end{tabular}
% s}
\vspace{-2ex}
\label{tab:fsl}
\end{table}



%\paragraph{Benchmark.} We trained ~\citep{sauder2019self} (Jigsaw) on ModelNet40 and reported in all.
% We compare with~\citep{sharma2020self} in the few-shot settings.
% \textit{\abbrev Pre-training configurations}: 
% %transferability we will only  The dataset for the pretrained completion tasks are based on either ShapeNet \cite{yuan2018pcn} or ModelNet40. %(as we described the construction process in the previous sections). 
% We use the 3D computer graphics software, Blender~\cite{blender}, to generate occluded point clouds. 
% %Then we use eq. \ref{eq:world_transform} to restore the occluded point cloud from the depth images, each pixel in the depth image is correspondent to a spatial point in the occluded point cloud. 
% For the ShapeNet dataset, we consider 
% %we use the data provided by \cite{yuan2018pcn}, which contains
% 30974 objects from 8 categories for pre-training. For each object we generate 8 occluded point clouds from randomly chosen viewpoints. The camera is set to 100, 120 and 160 units for focus, height and width, respectively, of the rendered depth images. The average number of points for each object is around 1000, which is more coarse compared with our pre-processed dataset based on ModelNet40.

% The top half of the table reports results for eight randomly initialized point cloud models, while the bottom-half reports results on two models across three pre-training methods.
\begin{table*}[t!]\small
\centering
\vspace{-1ex}
\caption{Mean point accuracy (mAcc) and intersection of union (mIoU) on ShapeNetPart. We reported the mean and std over three runs.}
% As in Table 2, `*' marks previously reported scores, and \textcolor{blue}{blue} and \textbf{bold} are best scores.
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
mAcc & 92.8$\pm$0.9 & 93.1$\pm$0.5 & \textcolor{blue}{93.4$\pm$0.7} & 92.3$\pm$1.0 & 92.6$\pm$0.9 & \textcolor{blue}{93.0$\pm$0.9} & 92.2$\pm$0.9 & 92.7$\pm$0.9 & \textbf{94.4$\pm$0.7} \\\hline
mIoU & 82.2$\pm$2.4 & 82.2$\pm$2.8 & \textcolor{blue}{83.4$\pm$1.9} & 81.3$\pm$2.6 & 81.2$\pm$2.9 & \textcolor{blue}{82.3$\pm$2.4} & 84.4$\pm$1.2 & 84.3$\pm$1.2 & \textbf{85.0$\pm$1.0} \\
\toprule
\end{tabular}
\vspace{-1ex}
\label{tab:partseg_result}
\end{table*}

\begin{table*}[t!]\small
\centering
\vspace{-1ex}
\caption{Mean point accuracy (mAcc) and class intersection of union (mIoU) on the S3DIS averaged across six folds over three runs.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
mAcc & 78.2$\pm$0.7 & 80.1$\pm$1.2 & \textcolor{blue}{82.0$\pm$1.0} & 82.9$\pm$0.9 & 83.7$\pm$0.7 & \textbf{85.1$\pm$0.5} & 83.7$\pm$0.7 & 84.1$\pm$0.7 & \textcolor{blue}{84.6$\pm$0.5} \\\hline
mIoU & 47.0$\pm$1.4 & 52.6$\pm$1.9 & \textcolor{blue}{54.9$\pm$1.0} & 51.1$\pm$2.4 & 52.2$\pm$1.9 & \textcolor{blue}{53.4$\pm$2.1} & 54.9$\pm$2.1 & 55.6$\pm$1.4 & \textbf{58.0$\pm$1.7}\\
\toprule
\end{tabular}
\label{tab:seg_result}
\end{table*}



\subsection{Fine-Tuning Results \label{fine_tuning_results}}
\subsubsection{Few-Shot Learning \label{sec:fsl}}
The results of few-shot learning are shown in Table \ref{exp:few_shot_classification}. We find that our model outperforms a strong few-shot baseline \cite{sharma2020self}, while both methods can significantly outperform randomly-initialized baselines with different architectures. We therefore conclude that \abbrev can significantly improve the performance of few-shot learning.
\qi{Run few-shot on another dataset in future work}


\subsubsection{Object Classification Results}
\label{sec:classification}
In Table~\ref{tab:classification}, we compare OcCo with random and Jigsaw \citep{sauder2019self} initialization on three object classification datasets with three encoders. ``MN40'', ``ScN10'' and ``SO15'' stand for ModelNet40, ScanNet10 and ScanObjectNN respectively.  We show that OcCo-initialized models outperform the baselines on all the datasets. Especially, OcCo performs well not only on the in-domain dataset (MN40), but also on cross-domain datasets (ScN10 and SO15). The results are consistent across three encoders. These results demonstrate that the representations from \abbrev can transfer to object classification.


\qi{This can be put into the analysis section instead of saying it here: In appendix, we make more comparisons such as training a linear SVM based on the learned features from OcCo pre-training with other autoencoder and GAN based methods.} 

% We compare OcCo-initialized and randomly-initialized models on the object classification datasets. 
% For fine-tuning the downstream models, we use the settings in \cite{qi2017pointnet,wang2019dynamic}, for more details see Appendix~\ref{app:opt}.
 


% , increasing the absolute performance by as much as $33.1\%$ (on ShapeNet10 using the PointNet encoder). 
% The improvements are consistent across all the three encoder networks. 
% We conclude that \abbrev brings architecture-agnostic improvements compared to the random initialization on object classification. 
% \todo{ScanObjectNN(OBJ\_BG)}
%We initialize the weights of the classification model using the \abbrev pre-training weights as follows. We restore the encoder weight from the \abbrev model and then randomly initialize the remaining weights. %for layers with same scopes and shapes, then initialised the rest.
%For randomly initialized models, we initialize all the variables on the same network architecture. 
%We have observed that increasing the number of pre-training epochs does not monotonically improve performance. We discuss this further in Section~\ref{subsec:ss}. %Thus for classification, segmentation and few-shots learning tasks, we use the checkpoints that give the best training performance: 20 epochs with batch size of 64 for the pre-trained PCN-based models, and 10 epochs with batch size of 32 for the pre-trained PointNet-based models. 
%We repeated the training process for 3 times and reported the average in Table~\ref{tab:classification}. 

 %, including ShapeNet10, ScanNet10, ShapeNet Occluded and ScanObjectNN. 
%as well as the random initialised baseline (originally 92.2\%, now updated as 92.9\% in \cite{wang2019dynamic}), which shows the effectiveness of \abbrev compared to \cite{sauder2019self}. 

\subsubsection{Object Part Segmentation Results}
\label{sec:part_seg}
% We now compare \abbrev against prior initialization approaches on object classification tasks. 
% We compare OcCo-initialized and randomly-initialized models on the object classification datasets. 
% For fine-tuning the downstream models, we use the settings in \cite{qi2017pointnet,wang2019dynamic}, for more details see Appendix~\ref{app:opt}.
Table~\ref{tab:partseg_result} compares OcCo-initialization with random and Jigsaw \citep{sauder2019self} initialization on object part segmentation.
% , averaged across 3 trials.
We observe that OcCo-initialized models outperform or perform competitively in accuracy and IoU compared to the other two initializations. The results are consistent across three encoders. This demonstrates that \abbrev can improve object part segmentation, and the improvements are robust to different encoders. %(also in Figure~\ref{fig:tsne}).
% We reported the detailed scores on each individual shape class in the appendix, for total 15 classes, 

\subsubsection{Semantic Segmentation \label{sec:scene_seg}}
Here we compare random, Jigsaw and \abbrev initialization on semantic segmentation. We use $k$-fold cross validation following \citet{armeni20163d}.
% , i.e., split data into $k$-parts and train $k$ models where the test set is one of the $k$ folds and the train set is the remaining $k\!-\!1$ folds. 
%for each hold-out fold, we train a new model based on the examples from the other $k\!-\!1$ folds and test on the hold-out fold). % to produce training and testing sets. 
% During the training, we use a batch size of 24 and training epochs of 50. The learning rate is set as 1e-3 initially, decayed to half for every 300,000 iterations and then is clipped to ensure it does not drop below 1e-5.
The results are reported in Table \ref{tab:seg_result}. OcCo-initialized models outperform random and jigsaw-initialized ones, demonstrating that \abbrev pre-training can bring in significant improvements for semantic segmentation.\footnote{We notice that the best model in \citet{sauder2019self} (mIoU=41.2) underperforms the result in DGCNN~\cite{wang2019dynamic} (mIoU=56.1). They consider a transductive setting which is not directly comparable to ours, so here we stick to the supervised setting and report our reproduced scores. \qi{Cannot understand this sentence.}}

\section{Analysis}\label{subsec:probe-test}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{resources/PT.pdf}
    \caption{Visualisation on the learned features by OcCo-pretrained PointNet.}
    \label{fig:tsne}
\vspace{-1ex}
\end{figure*}
In this section, we perform extensive analyses to study the reasons for OcCo's success. We first show that \abbrev can improve sample efficiency and convergence in downstream tasks. Then, we use three techniques, including semantic concept detection, unsupervised mutual information probe and visualization, to demonstrate that a model pre-trained with \abbrev can extract rich and discriminative point cloud features even without fine-tuning. 

%  Since point cloud encoders usually learn each point feature either independently or via neighborhood aggregation, the feature maps usually do not change in the vertical direction (see Figure~\ref{fig:tsne}). Therefore we can skip the \emph{retrieval} step and directly quantify the alignment between
\qi{Why use ModelNet for sample efficiency experiment? The setting is a bit weird. This assumes that the downsteam task is in the same domain as the pre-training data. todo: test on another dataset, e.g. Shapenet for sample efficiency. Then report the results on both modelnet and another dataset for sample efficiency. The results on Pointnet do not seem very well. Maybe remove that part.}
\paragraph{Sample Efficiency.} We investigate whether \abbrev pre-training can improve sample efficiency in downstream tasks. To this end, we randomly select 1\%, 5\%, 10\% and 20\% of samples from training set for fine-tuning. The fine-tuned models are evaluated on full test set. As shown in Table \ref{tab:few_shot}, models with \abbrev pre-training achieve better results compared to models with either random or Jigsaw initialization, which confirms the effectiveness of OcCo pre-training for boosting sample efficiency. 

\qi{The ModelNet figures are from the sample efficiency experiments, which is a bit weird compared to the others, e.g. S3DIS, which is full set}
\paragraph{Convergence.} We study the effect of pre-training on convergence in downstream tasks. We plot learning curves during fine-tuning. The results for classification (ModelNet and ScanObjectNN) and segmentation (S3DIS) are shown in Figure~\ref{fig:learning_curves}. We observe that the models with \abbrev initialization converge faster and better than the models with random or  Jigsaw initialization. This shows that \abbrev pre-training can improve convergence in downstream tasks.

% For ScanObjectNN with DGCNN encoder, the OcCo-initialized model converges around 20 epochs and to a better test accuracy than the random and Jigsaw-initialized model. 
\begin{table}[t!]\small
\centering
\setlength{\tabcolsep}{4pt}
\caption{Sample efficiency with randomly, Jigsaw and OcCo-initialized models on ModelNet40. We use 1\%, 5\%, 10\% and 20\% of the training data and evaluate the model on the full test set.} %\abbrev initialization uses models pre-trained on the occluded dataset from ModelNet40.}
\begin{tabular}{c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{Baseline} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-7}
 & Rand & Jigsaw & \abbrev&  Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
1\%  & 56.9 & 55.7 & \textcolor{blue}{58.1} & 60.0 & 59.9 & \textbf{60.5} \\\hline
5\%  & 73.9 & 74.3 & \textcolor{blue}{74.9} & 79.4 & 79.2 & \textbf{79.7} \\\hline
10\% & 80.6 & \textcolor{blue}{81.3} & 81.1 & 84.4 & 84.4 & \textbf{84.5} \\\hline
20\% & 83.6 & \textcolor{blue}{84.2} & \textcolor{blue}{84.2} & 86.5 & 86.7 & \textbf{87.2} \\ %\hline %\hline
\toprule
\end{tabular}
\vspace{-3ex}
\label{tab:few_shot}
\end{table}
\begin{figure}[h!]
    \centering
     \includegraphics[width=0.5\textwidth]{resources/learning_curve_short.pdf}
     \vspace{-3ex}
     \caption{Learning curves of random, Jigsaw and OcCo-initialised models on fine tuning tasks.}
     \label{fig:learning_curves}
     \vspace{-1ex}
\end{figure}

\paragraph{Detection of semantic concepts.} We adopt \emph{network dissection}~\citep{bau2017network,bau2020understanding} to study whether \abbrev-pretrained models without fine-tuning can learn semantic concepts in an unsupervised fashion. Specifically, for each point cloud, network dissection first creates a binary mask $M_k$ based on the feature map from the $k$-th channel. If the activation of a point in the feature map is larger than a threshold, its mask value is 1. Otherwise its mask value is 0. $M_k$ is compared with the $n$-th concept mask $C_n$, which comes from ground-truth segmentation labels, e.g.\ the concept mask value is 1 if it belongs to an object part like the leg of a chair. Given a set of point clouds $\mathcal{D}_\mathcal{P}$, these masks are used to calculate the mean intersection of union (mIoU):
\begin{gather}
    \text{mIoU}_{(k, n)}=
    \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}
    \left[\frac{\left|M_{k}(\mathcal{P}) \cap C_{n}(\mathcal{P})\right|}
    {\left|M_{k}(\mathcal{P}) \cup C_{n}(\mathcal{P})\right|}\right]
\end{gather}
where  $|\cdot|$ is the set cardinality. Network dissection calculates the expectation of the intersection of the two masks divided by the union of the two masks. $\text{mIoU}_{(k, n)}$ can be interpreted as how well channel $k$ detects the concept $n$. In Figure~\ref{fig:feat-det}, we plot the number of concepts detected by either Jigsaw or \abbrev. \abbrev outperforms Jigsaw in terms of the total number of detected concepts. This demonstrates that pre-training with \abbrev can unsupervisedly learn semantic concepts.

\begin{figure}
    \centering
     \includegraphics[width=0.45\textwidth]{resources/learned_feat_short.pdf}
     \vspace{-3ex}
     \caption{Visualisation of detected concepts (e.g., chair backs, car wheels and headset bands) from the OcCo-initialised PointNet. Parts marked by blue are based on the generated binary mask from the specified unit, the green ones are annotated as the ground truth. \qi{Put this visualization to corresponding sections}}
    %  \label{fig:learning_curves}
     \vspace{-1ex}
\end{figure}

\begin{table*}[h]\small
\centering
\vspace{-1ex}
\caption{Adjusted mutual information (AMI) under transformations. We reported the mean and standard deviation over 10 random initialisation. Under the `transformation' column, `J', `T', `R' represent jittering, translation and rotation respectively.}
% \vspace{-2ex}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\bottomrule \multicolumn{3}{c|}{Transformation} & \multicolumn{4}{c|}{ShapeNet10} & \multicolumn{4}{c}{ScanObjectNN} \\ \hline
J & T & R & VFH & M2DP & Jigsaw & \abbrev & VFH & M2DP & Jigsaw & \abbrev \\ \toprule \bottomrule
& & & 0.12$\pm$0.01 & 0.22$\pm$0.03 & 0.33$\pm$0.04 & \textbf{0.51$\pm$0.03} & 0.05$\pm$0.02 & 0.18$\pm$0.02 & 0.29$\pm$0.02 & \textbf{0.44$\pm$0.03} \\\hline
\checkmark & & & 0.12$\pm$0.02 & 0.19$\pm$0.02 & 0.32$\pm$0.02 & \textbf{0.45$\pm$0.02} & 0.06$\pm$0.02 & 0.17$\pm$0.02 & 0.27$\pm$0.02 & \textbf{0.42$\pm$0.04} \\\hline
\checkmark & \checkmark & & 0.13$\pm$0.03 & 0.21$\pm$0.02 & 0.29$\pm$0.07 & \textbf{0.38$\pm$0.04} & 0.04$\pm$0.02 & 0.18$\pm$0.03 & 0.24$\pm$0.04 & \textbf{0.39$\pm$0.06} \\\hline
\checkmark & \checkmark & \checkmark & 0.07$\pm$0.03 & 0.20$\pm$0.04 & 0.28$\pm$0.03 & \textbf{0.35$\pm$0.05} & 0.04$\pm$0.01 & 0.16$\pm$0.03 & 0.18$\pm$0.09 & \textbf{0.34$\pm$0.06} \\\hline
\toprule
\end{tabular}
\label{tab:so3}
\end{table*}
\vspace{3ex}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=1\textwidth]{resources/Feat_Det_Full.pdf}
    % \includegraphics[width=1\textwidth]{resources/Feat_Det_Short.pdf}
    \vspace{-3ex}
    \caption{Number of (unique) detected object parts in the `Feat1'~(above), `Feat2'~(middle) and `Feat3'~(below) module of Jigsaw and OcCo-initialised PointNet feature encoder. Digits in the bracket are the number of parts in that object category.}
    \label{fig:feat-det}
\end{figure*}

\paragraph{Unsupervised mutual information probe.} We hypothesize that a pre-trained model without fine-tuning can learn label information in an unsupervised fashion. For validation, we take PointNet pretrained with ModelNet40 to extract features for ShapeNet10 and ScanObjectNN. Then, we cluster the features with an unsupervised clustering method, K-means (where K is set to the number of ground-truth labels). To evaluate the quality of clustering, we calculate the adjusted mutual information (AMI)~\citep{nguyen2009information} between the predicted clusters and the ground-truth clusters obtained with class labels. AMI is 1 if these two clusterings are identical, while it has an expected value of 0 for a random clustering. Besides, we also study whether the pre-trained PointNet is robust to input transformations. In particular, we consider three transformations, including rotation, translation and jittering. Therefore, we apply these transformations to an input point cloud, before using PointNet to extract its features for clustering. 

We compare Jigsaw, \abbrev and two hand-crafted point cloud global descriptors: viewpoint feature histogram (VFH)~\citep{rusu2010fast} and M2DP~\citep{he2016m2dp} in Table~\ref{tab:so3}. We observe that pre-training methods, e.g.\ Jigsaw and \abbrev, can learn more discriminative feature representations compared to handcrafted descriptors, while the representations from \abbrev are more predictive than Jigsaw. These results demonstrate that \abbrev is an effective approach for unsupervised feature learning.

%We show that \abbrev pre-training helps the networks to learn better embeddings of point cloud objects, especially when they are occluded and with outlier points (ScanObjectNN).


%We use  based on the clustering $\Omega$ and the ground truth label $\mathcal{C}$, 


% Based on normalised mutual information (NMI), 
%Therefore it allows direct comparisons between different datasets:
%\begin{gather}
%    \mathrm{AMI}(\Omega, \mathcal{C}) = 
%    \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}
%    \left[\frac{\mathrm{I}(\Omega; \mathcal{C})- \mathbb{E}[\mathrm{I}(\Omega; \mathcal{C})]}{(\mathrm{H}(\Omega)+\mathrm{H}(\mathcal{C}))/2- \mathbb{E}[\mathrm{I}(\Omega;\mathcal{C})]}\right]
%\end{gather}
%where $\Omega$ is the clustering determined by the learned embeddings $\mathrm{Enc}(\cdot)$ and unsupervised clustering methods such as K-means. $\mathrm{I}(\Omega ; C)=\sum_{k} \sum_{j} P\left(w_{k} \cap c_{j}\right) \log \frac{P\left(w_{k} \cap c_{j}\right)}{P\left(w_{k}\right) P\left(c_{j}\right)}$ denotes the mutual information, $\mathrm{H}(\cdot)$ is the entropy. 

%It is calculated as:
%\begin{gather}
%    \mathcal{L} = \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P},\mathcal{S}\sim \mathrm{SO(3)}}\left[\operatorname{AMI}(\Omega, \mathrm{Enc}(\mathcal{S}(\mathcal{P})))\right]
%\end{gather}





% $\text{mIoU}_{(k, n)}=\mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}(\mathrm{IoU}(M_{k}(\mathcal{P}), C_{n}(\mathcal{P}))) > 0.5$. 
% For random and pre-trained encoders, we counts the number of detectors over all features and concepts. 

% For NMI, we compare the performance of the clustering methods based on i) coordinates ii) coordinates + learned features.

% The calculation of the expectation $ \mathbb{E}[\mathrm{I}(\mathcal{C}; \mathcal{C}')]$ is provided in ~\citep{nguyen2009information}. 
%AMI has a maximal of 1 when two partitions are identical, and reaches a minimal of 0 if two clusters are total uncorrelated. 
% \paragraph{Invariance/Equivariance under SO(3) transformation}
% Similar with previous work~\citep{deng2018ppf}, we want the learned embeddings to be invariant or equivariant under rigid SO(3) transformations (i.e., rotation, translation, permutation). 

% where $d(\cdot, \cdot)$ is a distance metric such as $l2$ or cosine,  $\mathrm{Enc}(\cdot)$ is the pre-trained point cloud encoder. 
% Although single representation might vary after SO(3), we want the cluster structures to be preserved.
% We build up the partial point cloud datasets from either ShapeNet or ModelNet. The existed ShapeNet one is used by PCN and TopNet, and the ModelNet is created by ourselves with various resolutions which provide a coarse-to-fine scale for pretraining.
% Once we learn pre-trained \abbrev weights on the ModelNet40, we will demonstrate the encoder weights improve initialization over prior baselines for downstream tasks: object classification, object part and scene semantic segmentation, \emph{on any dataset}. This setup is challenging as the pre-training domain can be very different from the downstream domains. We detail the downstream tasks below.
%\paragraph{Probe test.} 


% For ModelNet40, we generate 10 occluded point clouds for each object from random viewpoints. 
% In order to assess representation transferability, we also use the ModelNet40 pre-training mechanism for training ScanNet10 models. Besides, we perform a more rigorous test of the transferability of pre-training datasets in Section 4.4).
%In order to test transferability of representations we do not 
%The camera's focus and rendered image width and height are 10 times that of the PCN, which provides the pretrained model a board and fine structured of 3D objects, and in section 4.4, we have shown that our dataset are better for the pretraining in terms of the performance of downstream tasks.



% \begin{table}[H]
% \centering
% \small
% \vspace{-2ex}
% \caption{Statistics of classification datasets}
% \vspace{-2ex}
% \begin{tabular}{l|c|c|c|c}
% \bottomrule 
% Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
% ModelNet40~\citep{wu20153d} & synthesized & 40 & 9,843 & 2,468 \\\hline
% ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
% ScanNet10~\citep{dai2017scannet} & real scanned & 10 & 6,110 & 1,769 \\\hline
% ScanObjectNN ~\citep{ScanObjectNN} & real scanned & 15 & 2,304 & 576 \\
% \toprule
% \end{tabular}
% \label{tab:so3}
% \vspace{-3ex}
% \end{table}

\paragraph{Visualisation of learned features.} We use visualization to explore what a pre-trained model without fine-tuning learn about point cloud features. In Figure~\ref{fig:tsne}, we visualize the features of the objects from test split of ModelNet40~\citep{46832}. We color the points according to their channel activations. If the activation is large, its color is dark. Otherwise the color is light. We find that, the pre-trained encoder is able to learn low-level geometric primitives, e.g., planes, cylinders and cones, in the early stage while the network recognises more complex shapes like wings, leafs and upper bodies. We further use t-SNE to visualize the features on ShapeNet10. We notice that distinguishable clusters are formed after pre-training. We therefore conclude that \abbrev can learn features that are useful to distinguish different parts of an object or a scene. These features will be beneficial to downstream tasks, e.g.\ object recognition and scene segmentation.

%is widely used to qualitatively understand the role of a convolutional neural network unit. It links highly activated parts of a CNN channel with human concepts which have semantic meaning. 

% We call channel $k$ a detector of concept $n$ when $\text{mIoU}_{(k, n)}$ is larger than a threshold value.

% \paragraph{Clustering on learned features for part segmentation}
% We can further analyse how helpful the learned features are
% % convex decompositions 
% on distinguishing semantic parts.
% % by comparing ACD with human part annotations on 400 shapes from ShapeNetPart, 
% We use clustering methods including K-means, spectral clustering and hierarchical agglomerative clustering (HAC) based on the coordinates of point clouds $\mathcal{P}_c$ fused w/wo learned features $\mathcal{F}_k$.
% % and approximate convex decompositions (ACD) based on the geometry of the point clouds $\mathcal{P}$.
% We set the number of clusters $N$ to be the amount of annotated parts in each shape $\mathcal{P}$. Given the set of $M$ parts $\mathcal{W}=\left\{w_{1}, w_{2}, \ldots w_{M}\right\}$ and the set of $N$ clusters $\mathcal{C}=\left\{c_{1}, c_{2}, \ldots c_{N}\right\}$, improved clustering performance is evaluated using differences in the normalized mutual information (NMI):
% \begin{gather}
%     \mathrm{NMI}(\mathcal{W}, \mathcal{C}) = \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}\left[\frac{\mathrm{I}(\mathcal{W}; \mathcal{C})}{(\mathrm{H}(\mathcal{W}) +  \mathrm{H}(\mathcal{C}))/2}\right]
% \end{gather}
% where $\mathrm{I}(\mathcal{W}; \mathcal{C})=\sum_{i=1}^{|\mathcal{W}|} \sum_{j=1}^{|\mathcal{C}|} P(w_i, c_j) \log \left(\frac{P(w_i, c_j)}{P(w_i) P(c_j)}\right)$ denotes the mutual information between classes $\mathcal{W}$ and clusters $C$, and $\mathrm{H}(\cdot)$ is the entropy. Better clusterings result in higher NMIs ($\in$ [0,1]).

% \paragraph{Clustering on learned embeddings for classification}


% \subsection{Learning Curves}
% \label{subsec:train_convergence}
% We plot the learning curves for classification and segmentation tasks in Figure~\ref{fig:learning_curves}. We observe that the models with \abbrev initialization converge faster to better test accuracy than the random and sometimes Jigsaw-initialized models. For example, on ModelNet40 with a PCN encoder, the OcCo-initialized model takes around 10 epochs to converge, while the randomly initialized model takes around 50 epochs. Similarly, for %S3DIS with PointNet encoder and 
% ScanObjectNN with DGCNN encoder, the OcCo-initialized model converges around 20 epochs and to a better test accuracy than the random and Jigsaw-initialized model. % large performance gains. 
%We conclude that \abbrev can 
%improve generalization and achieve better or comparable convergence speed on downstream tasks. 


==> OcCo ICCV 2021/sections/introduction.tex <==

Point clouds are a natural representation of 3D objects. 
% They are crucial for various real-world applications in robotics~\citep{yan2019data}, autonomous driving~\citep{li20173d, yue2018lidar}, and localization~\citep{elbaz20173d,angelina2018pointnetvlad}.
Recently, there has been a flurry of exciting new point cloud models in areas such as 
% semantic and instance 
segmentation~\citep{landrieu2018large,yang2019learning,hu2019randla} and object detection~\citep{zhou2018voxelnet,lang2019pointpillars,wang2020pillar}.
% , and scene reconstruction~\citep{li2016manhattan}. 
Current 3D sensing modalities (\textit{i.e.}, 3D scanners, stereo cameras, lidars) have enabled the creation of large repositories of point cloud data~\citep{Rusu_ICRA2011_PCL,hackel2017isprs}. However, annotating~point clouds is challenging as: (1) Point cloud data can be sparse and at low resolutions, making the identity of points ambiguous; (2) Datasets that are not sparse can easily reach hundreds of millions of points (e.g., small dense point clouds for object classification~\citep{zhou2013complete} and large vast point clouds for 3D reconstruction \citep{zolanvari2019dublincity});
(3) Labelling individual points or drawing 3D bounding boxes are both more complex and time-consuming compared with annotating 2D images~\citep{wang2019latte}.
Since most 
% deep learning 
methods require dense supervision, the lack of annotated point cloud data impedes the development of novel models.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{resources/occo2.pdf}
    \vspace{-3ex}
    % \caption{\method\, is a self-supervised pre-training method composed of two steps: (a) occlusion $o(\cdot)$ of an input point cloud $\mathcal{P}$ based on a random camera view-point into a partial point cloud $\tilde{\mathcal{P}}$, and (b) a model $c(\cdot)$ that completes the occluded point cloud $\bar{\mathcal{P}}$ so that $\bar{\mathcal{P}} \approx \mathcal{P}$. We demonstrate that the completion model $c(\cdot)$ can be used as initialization for downstream tasks (e.g., classification, segmentation) leading to faster training and better generalization over existing methods.}
    \caption{A simple method for point cloud pre-training: 1. Take any point cloud dataset and generate occluded point clouds for each input by  (a) randomly sampling a camera view-point, and (b) removing any points hidden from that view-point (for all experiments \emph{we use the same occluded dataset generated from ModelNet40}); 2. Train an encoder-decoder model to complete the occluded point clouds (the encoder can be any model that learns representations of point clouds, the decoder can be any completion model); 3. Use the learned encoder weights as initialization for any point cloud task (e.g., few-shot learning, object classification, part segmentation, semantic segmentation). Surprisingly, this method outperforms a variety of pre-training methods across multiple models and tasks.}
    %\caption{\abbrev  consists of two steps: (a) occlusion $o(\cdot)$ of a point cloud $\mathcal{P}$ based on a random camera view-point into a partial point cloud $\tilde{\mathcal{P}}$, and (b) a model $c(\cdot)$ that completes the occluded point cloud $\bar{\mathcal{P}}$ so that $\bar{\mathcal{P}} \approx \mathcal{P}$. We demonstrate that the completion model $c(\cdot)$ can be used as initialization for downstream tasks, leading to faster training and better generalization over existing methods.}
    \label{fig:overview}
    \vspace{-3ex}
\end{figure}


On the other hand, because of the rapid development of 3D sensors, unlabelled point cloud datasets are abundant. Recent work has developed unsupervised pre-training methods to learn initialization for point cloud models. 
These are based on designing novel generative adversarial networks (GANs)~\citep{wu2016learning,han2019view,achlioptas2017learning} and autoencoders~\citep{hassani2019unsupervised,li2018so,yang2018foldingnet}. However, completely unsupervised pre-training methods have been recently outperformed by the self-supervised pre-training techniques of \citep{sauder2019self} and \citep{alliegro2020joint}. Both methods work by first voxelizing point clouds, then splitting each axis into $k$ parts, yielding $k^3$ voxels. Then, voxels are randomly permuted, and a model is trained to rearrange the permuted voxels back to their original positions. The intuition is that such a model learns the spatial configuration of objects and scenes. 
However, such random permutation destroys all spatial information that the model could have used to predict the final object point cloud. 
% This potentially leads to prediction ambiguities: if two different objects have the same number of point cloud coordinates, then their random permutations are indistinguishable from each other. 

Our insight is that partial point-cloud masking is a good candidate for pre-training in point-clouds because of two reasons: (1) The pre-trained model requires spatial and semantic understanding of the input point clouds to be able to reconstruct masked shapes. (2) Mask-based completion tasks have become the \textit{de facto} standard for learning pre-trained representations in natural language processing (NLP) \citep{mikolov2013efficient,devlin2018bert,peters2018deep}. 
%been proven to be effective in learning pre-trained representations for language data. 
%This poses a number of practical limitations on learning. 1. Manual labeling of point cloud datasets for standard supervised learning problems is nearly always impractical (indeed annotating such datasets warrants a paper in its own right \cite{zolanvari2019dublincity}); 2. Models need to be carefully designed to allow for efficient training over such large datasets. Even models that have linear computation complexity in the dataset size must have small constant factors (e.g., few training epochs).
%and computer vision (CV) \cite{he2019momentum,chen2020simple} communities, %yet studies of self-supervised learning for point clouds are scarce, 
%we propose a novel pre-training mechanism, inspired by masked language modelling \cite{devlin2018bert}. % and shape completion \cite{yuan2018pcn} in CV. 
Different from random permutations, masking respects the spatial constraints that are naturally encoded in point clouds of real-world objects and scenes. Given this insight, we propose \emph{\method} (OcCo) a self-supervised pre-training method that consists of (a) a mechanism to generate occluded point clouds, and (b) a completion task to reconstruct the occluded point clouds. 

Specifically, in (a) point clouds are generated by determining what part of objects would be occluded if the underlying object was observed from a particular view-point. In fact, many point clouds generated from a fixed 3D sensor will have occlusions exactly like this. 
%The intuition is that point clouds collected in real-world will be like this.
% likely be in this way. 
Given an occluded point cloud, the goal of the completion task (b) is to learn a model that accurately reconstructs the missing parts of the point cloud. %The idea is that in order 
For a model to perform this task well, it needs to learn to encode localized structural information, based on the context and geometry of partial objects. % of a partial point cloud. 
This is something that is useful for any point cloud model to know, even if used only for classification or segmentation. 
%that is required to complete
%occlude portions of the point cloud, and learn a representation that can be used to accurately recreate the missing occluded points. Specifically, we generate occluded point-clouds by determining what points would be obstructed if the underlying object was observed from a particular view-point. 

We demonstrate that the weights learned by our pre-training method \emph{on a single unsupervised dataset} can be used as initialization for models in downstream tasks (e.g., object classification, part and semantic segmentation) to improve them, \emph{even on completely different datasets}. Specifically our pre-training technique:
%to improve generalization for object classification
%can obtain problem and domain-independent representations of point clouds. These representations have the following benefits:
%\begin{itemize}[leftmargin=*]
(i) leads to improved generalization over prior baselines on the downstream tasks of object classification, object part and scene semantic segmentation;  
(ii) speeds up 
%It transfers to different datasets: pre-training on one dataset improves task accuracy on others.
model convergence, in some cases, by up to $5\times$; 
(iii) maintains improvements as the size of the labelled downstream dataset decreases; 
(iv) can be used for a variety of state-of-the-art point cloud models.
% \footnote{Our code will be released upon acceptance.}

%\end{itemize}
% (a) improve generalization on downstream tasks, 
% (b) transfer to different datasets, 
% (c) reduce training time, even up to $5\times$, and 
% (d) are more effective than previous pre-training methods.

% We begin by reviewing major related work,
% on deep models for point clouds and pre-training techniques
% then detail our approach and show how it achieves state-of-the-art results in a fraction of typical training time.
% HERE
%only improve generalization on downstream tasks including classification and semantic segmentation, even on different datasets, but also speed up training.
%We propose an alternative self-supervised pre-training mechanism for point cloud models that we demonstrate addresses the lack of label information, improving generalization, and 
%HERE
%We demonstrate that by learning to reconstruct these partial point clouds, our model outperforms all other point-cloud initializations: improving generalization accuracy, and reducing training time for state-of-the-art models in some cases by an order of magnitude.

%     \2 Recent work that has attempted to learn improved initializations either:
%         \3 Can only be used in restrictive settings (GANs)
%         \3 Learn uninformed low-dimensional representations
%         \3 Destroy important spatial information
%To tackle the first problem, 


==> OcCo ICCV 2021/sections/method.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{resources/data_overview_new.pdf}
    \vspace{-2ex}
    \caption{Examples of generated self-occluded objects.}
    \label{fig:dataoverview}
\end{figure*}
We now introduce \method\,(OcCo). Our approach is shown in Figure~\ref{fig:overview}. Our main insight is that by continually occluding point clouds and learning a model $c(\cdot)$ to complete them, the weights of the completion model can be used as initialization for downstream tasks (e.g., classification, segmentation)
, speeding up training and improving generalization over other initialization techniques.
%procedures include two steps: occlusion, then completion. Occlusion is realized by rendering methods and completion is via deep learning based methods.


Throughout we assume point clouds $\mathcal{P}$ are sets of points in 3D Euclidean space, $\mathcal{P} = \{ p_1, p_2, ..., p_n \}$, where each point $p_i$ is a vector of coordinates $(x_i, y_i, z_i)$ and features (e.g. color and normal). 
We begin by describing the components that make up our occlusion mapping $o(\cdot)$. 
Then we detail how to learn a completion model $c(\cdot)$, giving pseudocode and the architectural details in appendix.
Finally we discuss the criteria on validating the effectiveness of a pre-training model for 3D point clouds.
% how helpful OcCo is  for various downstream tasks. 
% what we want from a pre-training tasks.
%We begin with an overview of the approach. We then review pinhole camera basics and how to specify view-points. We give our procedure for masking. We detail and give pseudocode for the completion task. Finally we give technical details we use to implement our approach.

%\subsection{Overview}
 
\subsection{Generating Occlusions}
\label{subsec:occ}
We first describe a randomized occlusion mapping $o: \mathbb{P} \rightarrow \mathbb{P}$ (where $\mathbb{P}$ is the space of all point clouds) from a full point cloud $\mathcal{P}$ to an occluded point cloud $\tilde{\mathcal{P}}$. %\footnote{Where $\mathbb{P}$ is the space of all point clouds.} 
We will do so by determining which points are occluded when the point cloud is viewed from a particular camera position. This requires three steps: 
(1) A projection of the point cloud (in a world reference frame) into the coordinates of a camera reference frame;
(2) Determining which points are occluded based on the camera view-points;
(3) Mapping the points back from the camera reference frame to the world reference frame. 
%We describe each of these in detail.

\paragraph{Viewing the point cloud from a camera.}
A camera defines a projection from a 3D world reference frame into a distinctive 3D camera reference frame. 
It does so by specifying a camera model and a camera view-point from which the projection occurs. 
The simplest camera model is the pinhole camera, and view-point projection for it 
% \footnote{In our experiments we will use a more sophisticated lens camera model. However, any camera model can be used. Thus, to avoid unnecessarily complicating the approach, we describe it in terms of the pinhole camera.}. 
%the projection for the pinhole camera 
is given by a simple linear equation:
%Specifically, this projection can be divided into two parts (a) a perspective projection into camera coordinate space, (b) a normalization by the third dimension. Part (a) is a linear projection that can be written as follows:
\begin{align}
    \begin{bmatrix}
    x_{\text{cam}} \\
    y_{\text{cam}} \\
    z_{\text{cam}} \\
    \end{bmatrix} = 
    \underbrace{\vphantom{
            \left[
                \begin{array}{ccc|c}
                r_1 & r_2 & r_3 & t_1 \\
                r_4 & r_5 & r_6 & t_2 \\
                r_7 & r_8 & r_9 & t_3
                \end{array}
            \right]}
        \begin{bmatrix}
        f & \gamma & w/2 \\
        0 & f      & h/2 \\
        0 & 0      & 1
        \end{bmatrix}}_{
            \substack{\text{intrinsic} \\ [ \;\;\;\; \mathbf{K} \;\;\;\; ]}}
    \underbrace{
        \left[
        \begin{array}{ccc|c}
        r_1 & r_2 & r_3 & t_1 \\
        r_4 & r_5 & r_6 & t_2 \\
        r_7 & r_8 & r_9 & t_3
        \end{array}
        \right]
    }_{\subalign{\text{rotation } &| \text{ translation} \\ [\;\;\;\mathbf{R}\;\;\;\;\; &| \;\;\;\;\;\;\;\mathbf{t}\;\;\;\;\;]}}
    \begin{bmatrix}
    x \\
    y \\
    z \\
    1 
    \end{bmatrix}.
    \label{eq:camera_transform}
\end{align}
In the above, $(x,y,z)$ are the original point cloud coordinates, the matrix including $r$ and $t$ entries is the concatenation of a 3D rotation matrix with a 3D translation vector, and the final matrix to the left is the camera intrinsic matrix ($f$ specifies the camera focal length, $\gamma$ is the skewness between the $x$ and $y$ axes in the camera, and $w,h$ are the width and height of the camera image). Given these, the final coordinates $(x_{\text{cam}},y_{\text{cam}},z_{\text{cam}})$ are the positions of the point in the camera reference frame. We will refer to the intrinsic matrix as $\mathbf{K}$ and the rotation/translation matrix as $[\mathbf{R} | \mathbf{t}]$.

%Part (b) is easily done by dividing $x_{\text{cam}},y_{\text{cam}}$ by $z_{\text{cam}}$. However, if we skip part (b) 


\paragraph{Determining occluded points.}
We can think of the point $(x_{\text{cam}},y_{\text{cam}},z_{\text{cam}})$ in multiple ways: (a) a 3D point in the camera reference frame; (b) a 2D pixel with coordinates $(f x_{\text{cam}}/z_{\text{cam}}, f y_{\text{cam}}/z_{\text{cam}})$ with a depth of $z_{\text{cam}}$. In this way, some 2D points resulting from the projection may be occluded by others if they have the same pixel coordinates, but appear at a larger depth. To determine which points are occluded, we first use \emph{Delaunay triangulation} to reconstruct a polygon mesh from the points, and remove the points which belong to the hidden surfaces that are determined via \emph{z-buffering}.

% However, because point clouds only sparsely cover object surfaces, we need a way to (i) approximate the surface of the point cloud, and then (ii) determine which points are hidden by these surfaces. To approximate the surface (i) we create a polygon mesh of the camera reference point cloud (e.g., via Delaunay triangulation). Solving (ii) is referred to in computer graphics as the problem of \emph{hidden-surface determination}.
% To solve this problem we use a well-known, highly-optimized technique called \emph{z-buffering}. Z-buffering, also referred to as depth-buffering, works by continually estimating the minimum depth of each image pixel in the camera reference frame. It starts with an initial depth buffer of infinite distance for each pixel. Then by looping over each polygon faces of the 3D object, and each pixel in each polygon, z-buffering checks if the depth of that pixel is less than the depth in the buffer. If it is, it updates the depth buffer with the smaller depth. Thus, cloud points at a certain pixel are occluded if all surrounding polygons are at depths greater than the depth of that pixel in the final depth buffer. We remove all these occluded cloud points.  %Z-buffering resolves overlap problems encountered in Painter's algorithm because it considers depth on a per-pixel basis in an order invariant way. 
%In practice, we use the efficient \emph{Blender} package to create meshes and perform z-buffering. 
%render the depth images based on the polygon mesh forms of objects in ModelNet40\cite{wu20153d}, which we will discuss more in Section~\ref{subsec:OcCo-Tech}.


%We briefly review ray tracing, the method we will use to define our randomized occlusion mapping $o(\cdot)$.
%\subsection{Masking via Self-Occlusion}
%\label{Subsec:masking}
%We describe a few representative methods for solving this problem, and how we will use them to construct our randomized mapping $o(\cdot)$.

% \paragraph{Painter's algorithm.}
% Arguably the simplest approach is Painter's algorithm. The idea is based on how a painter might draw a set of objects that overlap each other. Starting with the farthest objects, an artist draws objects that are increasingly closer, allowing the closer objects to overlap the farther ones. More specifically, the algorithm starts by rasterization: creating a polygon mesh for the point cloud (e.g., via Delaunay triangulation). It then computes the centroid of each polygon in the mesh, and sorts the polygons by the depth of their centroids. Then the algorithm loops over the polygons from farthest to closest. If a near polygon covers a more distant point cloud point $p$, that point is removed.
% %works by sorting all points by their depth and looping over them from farthest to closest. If a point $p$ occurs at the same pixel $(x_{\text{cam}},y_{\text{cam}})$ as another point $p'$, but at a closer depth, then the further point $p'$ is removed. 
% This process continues until all polygons are considered. 
% The strength of this approach is that all operations inside the main loop are extremely fast. The downsides of this method are (a) the complexity of sorting large numbers of points, and (b) if polygons overlap cyclically the algorithm can fail, unless polygons are adaptively broken.


% %A downside of z-buffering is that nearer dept

% \paragraph{Ray tracing.}
% %The idea behind ray casting is
% While ray tracing is a general rendering technique that can resolve object color in 2D images, it can also be used for hidden surface determination. The simplest algorithm for ray tracing, called ray casting, works by looping through each pixel and computing the ray that begins at the viewer's eye that goes through that pixel. Different from the above methods, it does not require a rasterized polygon mesh (although it can be used with one). Another popular idea is to fit local high-order polynomials between points in order to interpolate a surface between points \cite{levin2004mesh}. However a surface is generated, the closest surface that blocks the path of the ray can be determined through an intersection test. Finally points that are surrounded by surfaces that do not intersect any ray are hidden and are removed.
% Since the late 1980s there has been extensive work on speeding up ray tracing algorithms to achieve real-time ray tracing \cite{dykstra1987brl,wald2005interactive,mcguire2019introduction}. Because of this we opt for ray tracing as our approach for identifying view-point occlusions (although in principle any of the above methods can be applied).

%(3) Mapping the points back from the camera reference frame to word reference frame. 
\paragraph{Mapping back from camera frame to world frame.}
%\subsection{Mapping Back from Camera Frame to World Frame}
%Section~\ref{Subsec:masking} described how to obtain a self-occluded 3D object that is in the camera reference frame. In these 2.5D depth image, each pixel represents an small area, whose size depend on the rendering settings, from the surfaces of the objects. On the other hand, a point t from point cloud also represents a small area of the object surface. In practice, point clouds describing the synthesized CAD models are also sampled from the mesh faces \cite{qi2017pointnet,qi2017pointnet++}.
% However, if we directly tried to learn a point cloud completion model from these camera frame point clouds, the model would have to learn additional rotational/translational invariance to identify that the occluded point clouds are actually all versions of the same original point cloud. To allow the model to focus on learning more meaningful spatial relationships, 
Once occluded points are removed, we re-project the point cloud to the original world reference frame,
% . 
%Therefore, by explicitly mapping each pixel in the depth images back from camera frame to the original world frame, we can have point clouds representing self-occluded objects. 
% This can be done with,
via the 
% following 
inverse transformation of~\eqref{eq:camera_transform}.
% \begin{align}
%       \begin{bmatrix}
%     x' \\
%     y' \\
%     z' \\
%     1  \\
%     \end{bmatrix} = 
%     \underbrace{
%     \left[
%     \begin{array}{ccc|c}
%     r_1 & r_2 & r_3 & t_1 \\
%     r_4 & r_5 & r_6 & t_2 \\
%     r_7 & r_8 & r_9 & t_3 \\
%     0   &  0  & 0   &  1
%     \end{array}
%     \right]^\top
%     }_{\big[\subalign{\;\mathbf{R}\; &| \;\mathbf{t}\; \\ \boldsymbol{0}\; &| \;1}\big]^\top}
%     \underbrace{\begin{bmatrix}
%     1/f & -\gamma/f^2 & (\gamma h - f w)/(2 f^2) & 0 \\
%     0 & 1/f      & -h/(2f) & 0 \\
%     0 & 0      & 1 & 0 \\
%     0 & 0      & 0 & 1
%     \end{bmatrix}}_{\big[\subalign{\;\mathbf{K}^{-1}\; & \;\boldsymbol{0}\; \\ \boldsymbol{0}\;\;\;\;\; & \;1}\big]}
%     \begin{bmatrix}
%         x_{\text{cam}} \\
%         y_{\text{cam}} \\
%         z_{\text{cam}} \\
%         1
%     \end{bmatrix}.
%     \label{eq:world_transform}  
% \end{align}
%Here $\mathbf{K}^{-1}$ is the inverse camera intrinsic matrix and, because rotation matrices $\mathbf{R}$ are orthogonal, we have that $\mathbf{R}^{-1} = \mathbf{R}^\top$. Thus 
% Eq.~\eqref{eq:world_transform} is the linear transformation that most closely approximates the inverse of eq.~\eqref{eq:camera_transform}, producing point $(x',y',z')$ in the world frame. 
The randomized occlusion mapping $o(\cdot)$ is constructed as follows. Fix an initial point cloud $\mathcal{P}$.
% \footnote{During implementation, we center all point clouds in the world reference frame, and apply random rotations and translations on the camera} 
% but this is equivalent, right? does it matter whether we rotate in world or camera frame? gotcha
% it is :), just one more thing, ShapeNet Occuluded is the data provided in PCN, not created by us, otherwise it won't have issues as discussed in the appendix
% the issues in appendix C? D
% can we also mention this in the appendix?
% but they didn't create this as a dataset technically did they? or... I see I see
% okay  I can change this in the experiments
% so if it's alright could you move the footnote above to the appendix and I'll fix the ShapeNet description
% cool
% Done
% they do, I use the one they realeased
% yes, just remember somewhere saying that we create ShapeNet Occuluded, which is not
% the true implementation details are, we center the objects in 
Given a camera intrinsics matrix $\mathbf{K}$, sample rotation/translation matrices $[ [\mathbf{R}_1 | \mathbf{t}_1] , \ldots, [\mathbf{R}_V | \mathbf{t}_V]]$, where $V$ is the number of views. For each view $v \in [V]$, 
%\todo{we first align the center of $\mathcal{P}$ and the center of thee camera frame},
%since eq.1 and eq.2 has implicitly assume the camera centers at the origin of the world reference frame, so we need to make it clear 
% gotcha! I will say we assume all point clouds are centered
project $\mathcal{P}$ into the camera frame of that view-point using eq.~\eqref{eq:camera_transform}, find occluded points and remove them, then map the rest back to the world reference using its inverse.
% eq.~\eqref{eq:world_transform}. 
%using z-buffering. 
% We then solve the hidden surface determination problem (e.g., via ray tracing) to remove points that are occluded in that view-point. This produces a point-cloud in the camera frame. 
%Then we map pixels whose depths are not equal to the preset buffer layer depth back to the world frame using eq.~\eqref{eq:world_transform}. 
This yields the final occluded world frame point cloud for view-point $v$: $\tilde{\mathcal{P}}_v$.

\subsection{The Completion Task}
% introduce functions encodehat we are learning in this task
Given an occluded point cloud $\tilde{\mathcal{P}}$ produced by $o(\cdot)$, the goal of the completion task is to learn a completion mapping $c: \mathbb{P} \rightarrow \mathbb{P}$ from $\tilde{\mathcal{P}}$ to a completed point cloud $\overline{\mathcal{P}}$. %Let $\tilde{\mathcal{P}} \sim o(\Pc)$ refer to a single random draw yielding an occluded point cloud. 
We say that a completion mapping is accurate w.r.t. loss $\ell(\cdot,\cdot)$ if $\mathbb{E}_{\tilde{\mathcal{P}} \sim o(\Pc)} \ell( c(\tilde{\mathcal{P}}), \Pc ) \rightarrow 0$.
The structure of the completion model $c(\cdot)$ is an ``encoder-decoder" network~\citep{3D-EPN,yuan2018pcn,Tchapmi_2019_CVPR,WangAL20}. The encoder maps an occluded point cloud to a vector, and the decoder reconstructs the full shape. After pre-training, the encoder weights can be used as initialization for downstream tasks. In appendix we gives pseudocode for OcCo and describes the architectures.




% \subsection{Point Cloud Encoder}
% Our pre-training method can work with any architecture that gives a representation $\mathbf{h}_{\mathcal{P}}$ for each point cloud $\mathcal{P}$. 
% As most modern deep learning models for point clouds output either a global point cloud representation or local pointwise representations, our method can be integrated with previous models with ease, where the local pointwise representations are aggregated using symmetric functions (e.g. max pooling) for obtaining $\mathbf{h}_{\mathcal{P}}$. 

% \subsection{Shape Completion Network}
% The shape completion network takes the representation $\mathbf{h}_{\mathcal{P}}$ of the partial point cloud as input and generates a set of points for completion. We adopt a two-stage point generation scheme following PCN \cite{yuan2018pcn}. The two-stage point scheme uses the fully-connected decoder \cite{achlioptas2017learning} to generate a sparse set of points for determining the global geometry first, then applies the folding-based decoder \cite{yang2018foldingnet} for approximating a smooth surface around the points in the sparse set.

% More specifically, a sparse set $Y_{MLP}$ of $s$ points is generated by feeding $\mathbf{h}_{\mathcal{P}}$ to a multi-layer perceptron with $3s$ output units, i.e $Y_{MLP} = \mathrm{MLP}( \mathbf{h}_{\mathcal{P}} )$. The output vector is reshaped into a matrix of size $s \times 3$, where each column represents the 3D coordinates of a point. Then, for each point $p_i$ in $Y_{MLP}$, a set $Y^i_{FOLD}$ of $u^2$ points (in a local coordinate system with $p_i$ as the origin) are generated through the folding operation \cite{yang2018foldingnet}. Every point $p_j$ of the $u^2$ points is added with $p_i$ to map it to a global coordinate system, \textit{i.e.} $p_i + p_j$. As a result, a set $Y_{FOLD}$ with $u^2 \times s$ points is obtained after taking a union of $Y^i_{FOLD}$, \textit{i.e.} $Y_{FOLD} = \cup_i Y^i_{FOLD} $. 

% \subsection{Order-Invariant Loss Functions}
% For the shape completion task, the loss function measures the differences between the generated point clouds $\mathcal{P}_1$ and ground truth point clouds $\mathcal{P}_2$. As the points in a point cloud are unordered, the loss function needs to be permutation invariant. To this end, we adopt Chamfer Distance (CD) and Earth Mover's Distance (EMD): 

% \begin{equation}
%     \mathrm{CD}(\mathcal{P}_1, \mathcal{P}_2) = \frac{1}{|\mathcal{P}_1|} \sum_{p_i \in \mathcal{P}_1} \min_{y \in \mathcal{P}_2} \Vert p_i - y \Vert_2 + \frac{1}{|\mathcal{P}_2|} \sum_{p_i \in \mathcal{P}_2} \min_{x \in \mathcal{P}_1} \Vert p_i - x \Vert_2.
%     \label{eq:cd_distance}
% \end{equation}
% CD calculates the average closest point distance between $\mathcal{P}_1$ and $\mathcal{P}_2$. The symmetric version of CD is used in Equation \ref{eq:cd_distance} to ensure that $\mathcal{P}_1$ is close to $\mathcal{P}_2$, while the points in $\mathcal{P}_2$ are covered by the points in $\mathcal{P}_1$. CD can be computed with $O(n \log n)$ complexity using efficient $k$-nearest neighbor algorithms (e.g. KDTree).

% \begin{equation}
%     \label{eq:emd_distance}
%     \mathrm{EMD}(\mathcal{P}_1, \mathcal{P}_2) = \min_{\phi: \mathcal{P}_1 \rightarrow \mathcal{P}_2} \frac{1}{|\mathcal{P}_1|} \sum_{p_i \in \mathcal{P}_1} \Vert p_i - \phi(p_i) \Vert_2.
% \end{equation}
% EMD finds a bijection function $\phi: \mathcal{P}_1 \rightarrow \mathcal{P}_2$ that minimizes the average distance between corresponding points in $\mathcal{P}_1$ and $\mathcal{P}_1$. As finding the optimal $\phi$ is computationally-expensive in practice, the iterative $(1 + \epsilon)$ approximation scheme is applied \cite{bertsekas1985distributed}. EMD with the $(1 + \epsilon)$ approximation scheme can be computed with $O(n^2)$ complexity. Empirically we have shown that both loss functions are effective in terms of performance gains of the downstream tasks.

% As we adopt the two stage generation scheme, we use the following loss function:

% \begin{equation}
%     \label{eq:loss}
%     L(Y_{MLP}, Y_{FOLD}, Y) = \mathrm{EMD}(Y_{MLP}, \hat{Y}) + \mathrm{CD}(Y_{MLP}, \hat{Y}) + \alpha \mathrm{CD}(Y_{FOLD}, Y),
% \end{equation}
% where $Y$ is the occluded set of points and $\hat{Y}$ is a sub-sampled set of points to serve as the ground truth for the sparse set $Y_{MLP}$. We did not include $\mathrm{EMD}(Y_{FOLD}, Y)$ here due to the $O(n^2)$ complexity of the earch mover's distance. $\alpha$ is a hyperparameter.


==> OcCo ICCV 2021/sections/related.tex <==
%!TEX root = ../main.tex
\qi{draw a figure summarizing previous pretrainign work. which dataset they used. it is object/scene pretraining? The fine-tuning tasks and datasets.}
% omit this, and cite a review paper
\subsection{Deep Models for Point Clouds}

Work on deep models for point clouds can largely be divided into three different structural approaches: (a) \emph{pointwise-based networks}, (b) \emph{convolution-based networks}, and (c) \emph{graph-based networks}.
We call the networks that independently process each point, before aggregating these point representations: \emph{pointwise-based networks} \citep{qi2017pointnet,qi2017pointnet++,joseph2019momen,duan2019structural,zhao2019pointweb,yang2019modeling,lin2019justlookup}. One well-known method, PointNet, devises a novel neural network that is designed to respect the permutation invariance of point clouds. Each point is independently fed into a multi-layer perceptron, then outputs are aggregated using a permutation-invariant function (e.g., max-pooling) to obtain a global point cloud representation.
% Two well-known models of this type are PointNet and PointNet++. PointNet \cite{qi2017pointnet} devises a novel neural network that is designed to respect the permutation invariance of point clouds. Each point is independently fed into a multi-layer perceptron, then outputs are aggregated using a permutation-invariant function (e.g.,  max-pooling) to obtain a global point cloud representation. However, as PointNet does not capture local structures induced by the 3D metric space, PointNet++ \cite{qi2017pointnet++} extends it by partitioning the point sets into overlapping local regions via a distance metric. It recursively groups local features into larger units to produce higher-level features. 
Another class of methods are \emph{convolution-based networks} \citep{hua2018pointwise,su2018splatnet,li2018pointcnn,atzmon2018point,landrieu2018large,hermosilla2018monte,groh2018flex,rao2019spherical}. These works map point clouds to regular grid structures and extend the classic convolution operator to handle these grid structures. 
%\paragraph{Convolution-based networks.}
%We call the networks that map point clouds to regular grid structures and extend the classic convolution operator to handle these grid structures as convolution-based networks \cite{hua2018pointwise,su2018splatnet,li2018pointcnn,atzmon2018point,landrieu2018large,hermosilla2018monte,groh2018flex,rao2019spherical}. 
A representative model, PCNN \citep{atzmon2018point}, defines two operators, extension and restriction, for mapping point cloud functions to volumetric functions and vise versa.
%To describe how models of this type function, we highlight four representative models: SPLATNet \cite{su2018splatnet}, PointCNN \cite{li2018pointcnn}, PCNN \cite{atzmon2018point} and SPG \cite{landrieu2018large}. SPLATNet \cite{su2018splatnet} maps points onto a sparse lattice, and then performs bilateral convolution only on parts of the lattice that are occupied by points. PointCNN \cite{li2018pointcnn} determines a canonical point ordering by learning a permutation and weighting of points, called an $\mathcal{X}$-transformation, before applying a conventional convolution operator. PCNN \cite{atzmon2018point} defines two operators, extension and restriction, for mapping point cloud functions to volumetric functions and vise versa. SPG \cite{landrieu2018large} focuses on dealing with large point clouds, where a superpoint graph is constructed by adaptively partitioning points into geometrically homogeneous elements. The superpoint graph is then fed into a graph neural network to produce its corresponding semantic labels. 
The third class of models is \emph{graph-based networks} \citep{simonovsky2017dynamic,wang2019dynamic,shen2018mining,wang2018local,zhang2018graph,chen2019clusternet}. These networks regard each point as a vertex of a graph and generate edges based on spatial information and node similarities. 
%as graph-based networks  \cite{simonovsky2017dynamic,wang2019dynamic,shen2018mining,wang2018local,zhang2018graph,chen2019clusternet}. 
A popular method is DGCNN \citep{wang2019dynamic}, which introduces a new operation, EdgeConv, to aggregate local features and a graph update module to learn dynamic graph relations from layer to layer. NRS~\citep{NRS} uses a neural random subspace method based on the encoded embeddings to further improve the model performance.
%PointNet++ \cite{qi2017pointnet++} also falls into this category as it assumes a fixed local graph structure during training, and uses this to compute pairwise point distances. Other graph-based point cloud models include DGCNN \cite{wang2019dynamic}, which generalizes PointNet++ by introducing a new operation, EdgeConv, to aggregate local features and a graph update module to learn dynamic graph relations from layer to layer. PointGCN \cite{zhang2018graph} combines localized graph convolutions with two types of graph downsampling operations. ClusterNet \cite{chen2019clusternet} designs a hierarchical clustering network to obtain rotation-invariant representations. 
%\newline

%\noindent
%we propose a new pre-training method that can be used for any of the above existing architectures to accelerate training.
%that is applicable to existing architectures.
% HERERE

\subsection{Pre-Training for Point Clouds}
Pre-training models on unlabelled data are gaining popularity recently due to its success on a wide range of tasks, such as natural language understanding \citep{mikolov2013efficient,devlin2018bert}, object detection \citep{he2019momentum,chen2020simple} and graph representations \citep{hu2019pre,GPT}. 
The representations learned from these pre-trained models can be used as a good initializer in downstream tasks, where task-specific annotated samples are scarce. 
The three most common pre-training objectives for point clouds are based on:
(i) generative adversarial networks (GAN), (ii) autoencoders, and (iii) spatial relation. 
However, GANs for point clouds are limited to non-point-set inputs, i.e., voxelized representations~\citep{wu2016learning}, 2D depth images of point clouds \citep{han2019view}, and latent representations from autoencoders \citep{achlioptas2017learning}, as sampling point sets from a neural network is non-trivial. Thus these GAN approaches cannot leverage the natural order-invariance of point-sets. 
Autoencoders \citep{yang2018foldingnet,li2018so,hassani2019unsupervised,ShiXYF20} learn to encode point clouds into a latent space before reconstructing these point clouds from their latent representation. 
Similar to these methods, generative models based on normalizing flow~\citep{pointflow} and approximate convex decomposition~\citep{gadelha2020label} have been shown effective for the unsupervised learning on point clouds. 
% \todo{Yet, there is recent evidence that the representations learned by autoencoders are not necessarily good when used as initialization for downstream tasks~\citep{alberti2017pitfall}.}
However, both GAN and autoencoder-based pre-training methods have been recently outperformed on downstream tasks by the pre-training technique of~\citet{sauder2019self} or~\citet{sharma2020self} in few-shot setting.
%and \citet{alliegro2020joint}.

These methods are based on spatial relation reconstruction, %which can be seen as an extension of solving jiggle puzzles in 2D images \cite{NorooziF16}. 
which aims to reconstruct points clouds given rearranged point clouds as input. To this end, \citet{sauder2019self} equally split the 3D space into $k^3$ voxels, rearrange $k^3$ voxels and train a model to predict the original voxel label for each point. However, these random permutations destroy all spatial information that the model could have used to predict the true point cloud. 
Inspired by cover-trees~\citep{beygelzimer2006cover}, \citet{sharma2020self} utilised ball covers for hierarchical partitioning of points. They then train a model to classify each point to their assigned clusters. However, the selection of the ball centroids is somewhat random and they need to pre-train from scratch for each fine-tuning task. 
% \citep{alliegro2020joint} further developed this approach into % 3D puzzle solving task into a multi-task learning framework where other tasks are supervised, i.e. classification and part segmentation.
Instead, our method creates spatially realistic occlusions that a completion model learns to reconstruct. As such, this model learns how to naturally encode 3D object shape and contextual information. Recently there is a new method called PointContrast~\citep{pointcontrast} which mainly uses contrastive learning for pre-training indoor segmentation models. Our method is more general and transferable compared with theirs. 

Point cloud completion~\citep{yuan2018pcn} has received attentions in recent years. Most works aim at achieving a lower reconstruction loss by incorporating 1) a better encoder~\citep{xie2020grnet,huang2020pf}, 2) a better decoder~\citep{Tchapmi_2019_CVPR,wen2020point}; 3) cascaded refinement~\citep{WangAL20} and 4) multi-viewed consistency~\citep{hu20203d}.

Completing 3D shapes for model initialisation has been considered before. \citet{schonberger2018semantic} used scene completion~\citep{song2017semantic,dai2020sg,hou2020revealnet} as an auxiliary task to initialise 3D voxel descriptors for visual localisation. 
They generated nearly-complete and partial voxelised scenes based on depth images and trained a variational autoencoder for completion. They have showed that the pre-trained encoder is more robust under different viewpoints and weather conditions. %However, they do not explicitly show that the pre-training brings improvements since the lack of the control group (i.e., training from scratch.)
% SG-NN~\citep{dai2020sg} and RevealNet~\citep{hou2020revealnet} specifically tackles the unsupervised scene completion task  by inferring unobserved scene geometry. 
We adapt this idea to pre-training for point clouds. We have shown that our initialisation is better than random and prior methods in terms of 1) object understanding; 2) invariance under transformations; and 3) downstream task performance.
% based we show that such learned embeddings are also robust to transformation and 
% \todo{Compared to these works OcCo is different in a significant way: our approach only learn pre-trained weights on a single dataset (ModelNet40). We have shown that such pre-trained weights outperform all point cloud baselines in few-shot learning, improve generalization on many different classification tasks, and have better transformation invariance than prior work. As far as we are aware it was not known that such pre-training would yield such improvements across tasks and datasets.}
% Compared with these works, 
% in \abbrev, 
% On this basis, 
% we have provided more in-depth and interpretable analysis on the learned representations after pre-training as well as shown more transferable ability. 

%On the basis of these, we provide more in-depth analysis of the pre-training process with network dissection and invariance under SO(3) transformation. We further show that completing the occluded objects~\citep{yuan2018pcn,Tchapmi_2019_CVPR,WangAL20,WenLHL20} is transferable to improve the generalisation of various downstream tasks as well as label efficiency.
% However, our method show that the 3D completion task 
%Instead we propose a method utilizing the occlusion completion, where the objective directly takes point clouds as input and completes the partial point clouds based on spatial relations. Compared with Sauder and Sievers \cite{sauder2019self} and Alliegro et al.\cite{alliegro2020joint}, our method purely origins from the 3D vision perspective and achieves better results with the same baselines on both synthetic and real-world datasets. 
%In this paper, our goal is to propose a novel pre-training mechanism that can be used to learn initialization for any of the above architectures. These initialization will accelerate training and improve generalization.
%Before we describe our method, we review current work in pre-training methods for point clouds, their shortcomings, and how our approach will address these.

% \subsection{Pre-training for Images}
% Pre-training~(a.k.a. self-supervised learning) has been widely used on images. Inspired by the unsupervised method~\cite{mikolov2013efficient} from natural language processing domain which rely on predicting works from their context, ~\cite{doersch2015relative} proposed a practically successful pre-training task of predicting the relative location of image patches. After this work,~\cite{noroozi2016jigsaw} introduced a method predicting the permutation of a ``jigsaw puzzle'' which is created from the full images. In contrast to these patch-based methods, some methods generate cleverly designed image-level classification tasks. In~\cite{gidaris2018rotation}, an image is randomly rotated by one of four possible angles and let the model predict the rotation. Another class of pre-training tasks contains tasks with dense spatial outputs. Some examples are image colorization~\cite{zhang2016colorful}, split-brain autoencoders~\cite{zhang2017split}, image inpainting~\cite{pathak2016context}, and motion segmentation prediction~\cite{pathak2017learning}. 


==> OcCo ICCV 2021/sections/related_new.tex <==
%!TEX root = ../main.tex

% omit this, and cite a review paper
% The current developments in deep point cloud models can be referred to~\cite{9127813}.

Pre-training models on unlabelled data are gaining popularity recently due to its success on a wide range of tasks, such as natural language understanding \citep{mikolov2013efficient,devlin2018bert}, object detection \citep{he2019momentum,chen2020simple} and graph representations \citep{hu2019pre,GPT}. 
The representations learned from these pre-trained models can be used as a good initializer in downstream tasks, where task-specific annotated samples are scarce. 
The three most common pre-training objectives for point clouds are based on:
(i) generative adversarial networks (GAN), (ii) autoencoders, and (iii) spatial relation. 
However, GANs for point clouds are limited to non-point-set inputs, i.e., voxelized representations~\citep{wu2016learning}, 2D depth images of point clouds \citep{han2019view}, and latent representations from autoencoders \citep{achlioptas2017learning}, as sampling point sets from a neural network is non-trivial. Thus these GAN approaches cannot leverage the natural order-invariance of point-sets. 
Autoencoders \citep{yang2018foldingnet,li2018so,hassani2019unsupervised,ShiXYF20} learn to encode point clouds into a latent space before reconstructing these point clouds from their latent representation. 
Similar to these methods, generative models based on normalizing flow~\citep{pointflow} and approximate convex decomposition~\citep{gadelha2020label} have been shown effective for the unsupervised learning on point clouds. 
% \todo{Yet, there is recent evidence that the representations learned by autoencoders are not necessarily good when used as initialization for downstream tasks~\citep{alberti2017pitfall}.}
However, both GAN and autoencoder-based pre-training methods have been recently outperformed on downstream tasks by the pre-training technique of~\citet{sauder2019self} or~\citet{sharma2020self} in few-shot setting.
%and \citet{alliegro2020joint}.

These methods are based on spatial relation reconstruction, %which can be seen as an extension of solving jiggle puzzles in 2D images \cite{NorooziF16}. 
which aims to reconstruct points clouds given rearranged point clouds as input. To this end, \citet{sauder2019self} equally split the 3D space into $k^3$ voxels, rearrange $k^3$ voxels and train a model to predict the original voxel label for each point. However, these random permutations destroy all spatial information that the model could have used to predict the true point cloud. 
Inspired by cover-trees~\citep{beygelzimer2006cover}, \citet{sharma2020self} utilised ball covers for hierarchical partitioning of points. They then train a model to classify each point to their assigned clusters. However, the selection of the ball centroids is somewhat random and they need to pre-train from scratch for each fine-tuning task. 
Instead, our method creates spatially realistic occlusions that a completion model learns to reconstruct. As such, this model learns how to naturally encode 3D object shape and contextual information. Recently there is a new method called PointContrast~\citep{pointcontrast} which mainly uses contrastive learning for pre-training indoor segmentation models. \todo{add a few on contrastive works}
% Our method is more general and transferable compared with theirs. 

% Point cloud completion~\citep{yuan2018pcn} has received attentions in recent years. Most works aim at achieving a lower reconstruction loss by incorporating 1) a better encoder~\citep{xie2020grnet,huang2020pf}, 2) a better decoder~\citep{Tchapmi_2019_CVPR,wen2020point}; 3) cascaded refinement~\citep{WangAL20} and 4) multi-viewed consistency~\citep{hu20203d}.

Completing 3D shapes for model initialisation has been considered before. \citet{schonberger2018semantic} used scene completion~\citep{song2017semantic,dai2020sg,hou2020revealnet} as an auxiliary task to initialise 3D voxel descriptors for visual localisation. 
They generated nearly-complete and partial voxelised scenes based on depth images and trained a variational autoencoder for completion. They have showed that the pre-trained encoder is more robust under different viewpoints and weather conditions. %However, they do not explicitly show that the pre-training brings improvements since the lack of the control group (i.e., training from scratch.)
% SG-NN~\citep{dai2020sg} and RevealNet~\citep{hou2020revealnet} specifically tackles the unsupervised scene completion task  by inferring unobserved scene geometry. 
We adapt this idea to pre-training for point clouds. We have shown that our initialisation is better than random and prior methods in terms of 1) object understanding; 2) invariance under transformations; and 3) downstream task performance.


==> sections/abstract.tex <==
%There has recently been a flurry of exciting advances in deep learning models on point clouds. However, these advances have been hampered by the difficulty of creating labelled point cloud datasets: sparse point clouds often have unclear label identities for certain points, while dense point clouds are time-consuming to annotate. We describe a %%%% HERE
We propose a surprisingly simple pre-training approach for point clouds. Inspired by mask-based pre-training in the natural language processing community, it works in three steps: 1. Mask all points that are occluded in different camera views; 2. Learn an encoder-decoder model to reconstruct the occluded points; 3. Use the encoder weights  as initialization for any downstream task. Surprisingly, we find that even when we construct a single pre-training dataset (from ModelNet40), the pre-trained encoder improves accuracy on a wide range of downstream tasks, across different datasets and encoder models. Specifically, we show that this method is competitive with recent work in the few-shot learning setting. At the same time it improves final generalization accuracy in object classification, part and semantic segmentation tasks. To better understand this approach, we investigate the pre-trained weights using various probe tests and visualizations. Code is available at https://anonymous.

%It then optimizes a completion model that learns how to reconstruct the occluded points, given the partial point cloud. In this way, our method learns a pre-trained representation that can identify the visual constraints inherently embedded in real-world point clouds. 
%We call our method \emph{Occlusion Completion} (OcCo). 
%learns representations that improve the semantic understandings as well as generalization on downstream tasks over prior methods, %that
%transfer to different datasets, %that
%reduce training time and improve label efficiency.
% sample efficiency. 
% Our code and dataset are available at \href{https://github.com/hansen7/OcCo}{{\color{blue}https://github.com/hansen7/OcCo}}.


==> sections/discussion.tex <==
%!TEX root = ../main.tex
In this work, we have demonstrated that why and how the Occlusion Completion (OcCo) learns the representations on point clouds that are more transformation invariant, more accurate in few-shot learning, and in various classification and segmentation fine tuning tasks, compared to prior work.
% generalizable representations for a variety of point cloud learning tasks, while increasing labelled sample efficiency and model convergence speed. %Further, these representations accelerate training fully-supervised learning. 
% \todo{to reduce a few in the future works.}
% There are a few exciting directions that we would like to explore in future. 
% First, we believe this method would be useful as a data-augmentation technique during training to improve robustness, similar to input dropout in the 2D case \citet{bouthillier2015dropout}. 
%The idea is that if a model is still good at say, classification, from partial point clouds, it will likely generalize better to unseen point clouds. 
% Second, 
In future, 
it would be interesting to design a completion model that is explicitly aware the view-point of the occlusion. 
% that it is completing an occluded view-point. 
A model like this would likely converge even quicker, and require fewer parameters, as this knowledge could act as a stronger inductive bias during learning. 
%Third, we believe there are a host of other 3D computer graphics concepts that could be leveraged to learn improved representations %generalizable and computationally efficient representations 
%for point cloud data.  %Specifically, a model that tries to predict how polygon meshes of 3D point clouds cast shadows would likely have a generic understanding of the 3D object behind the point cloud. 
%Similarly, a model that learns how to distinguish incoming versus emitted spectral radiance of a 3D surface via a deep parameterization of the rendering equation would likely produce a representation that improves classification and segmentation. 
In general, we advocate for structuring deep models using graphical constraints as an inductive bias to improve learning.

% \paragraph{Acknowledgements}
% Hanchen would acknowledge the support from Cathy Xu Fellowship, Cambridge Trust Scholarship and CAPA Award, as well as Cambridge Engineering technician team.

==> sections/experiments.tex <==
\newcommand{\qi}[1]{\textcolor{green}{\bf [Qi: #1]}}
\qi{1. Change standard deviation to standard error. 2. We color \textcolor{blue}{blue} the best results for each encoder and \textbf{bold} in black the overall best result for each dataset. 3. tidy the appendix section. }
%!TEX root = ../main.tex
% \begin{figure}[t!]
%     \centering
%     \vspace{-7ex}
%     \includegraphics[width=.9\linewidth]{resources/occlusion_steps.pdf}
%     \vspace{-1ex}
%     \caption{Overview of the procedure to generate occluded point clouds. See text for details.}
%     \label{fig:occlusion_steps}
%     \vspace{-2ex}
% \end{figure}

% We evaluate \abbrev on various downstream tasks, models, and datasets. 
%In Section \ref{sec:pretrain_settings}, we present the datasets and pre-training settings. We then show results on object classification tasks in Section \ref{sec:classification}, and semantic segmentation in Section \ref{sec:scene_seg}. In Section \ref{sec:efficiency}, we demonstrate that in cases where labelled data is particularly sparse, our method boosts accuracy. Related to this, models with \abbrev initialization converge faster to better test accuracies than randomly initialized models, which we show in Section~\ref{subsec:train_convergence}. Finally, we present further results on the sensitivity of our model to hyperparameter choices in the appendix. 
% All experiments are conducted on a 8-core NVIDIA GTX 1080 cluster and a 10-core NVIDIA RTX 6000 cluster.
%\abbrev improves sample efficiency. More experiments are presented in the appendix.

%our method improves representation learning with faster convergence speed and better scores. Then we investigate how our method perform when providing less training data.
%and finally we evaluate how sensitive our model is to the settings of \abbrev pre-training. 
% We then evaluate the transferability of the learned representations, and how they affect training convergence. 
% Finally, we demonstrate our method improves learning with less training labels, 

%In the appendix, we also include how we choose which weights from the \abbrev pre-training to be restored for the downstream tasks, and the difference between our constructed self-occluded point cloud data based on ModelNet40 and the other one based on ShapeNet which is used in the previous work\cite{yuan2018pcn,Tchapmi_2019_CVPR,abs-2004-03327} on point cloud completion.

In this section, we first present the details of OcCo pre-training (Section \ref{sec:pretrain_settings}), and fine-tuning (Section \ref{fine_tuning_details}). The results of few-shot learning, object classification, part segmentation and semantic segmentation are shown in Section \ref{fine_tuning_results}.


\subsection{OcCo Pre-Training Details \label{sec:pretrain_settings}}

% We now describe the datasets, models, and tasks we use for evaluation.
% of \abbrev.

%\textit{\abbrev pre-training details}: %For the occlusion completion pretraining tasks, we use PCN and PointNet to encode the global features of the occluded point cloud, and the two-stage decoder to generate the coarse and fine completed point cloud. Each object is normalised into unit sphere and repeatedly sampled or downsampled into 1024 points, the number of points in the coarse and detailed outputs are 1024 and 16384 respectively.
% some of the examples are visualised in Figure.~\ref{fig:dataoverview}.

% \todo{Add More, as in the Commented Paragraphs. Maybe put the architecture details into appendix and refer to it?}

% \subsection{Technical Details}
% We first describe how we generate the occluded point clouds. The intrinsics of the camera (in eq.~\ref{eq:camera_transform}) are set to $f=1000, \gamma=0, \omega=1600, h=1200$. For each polygon mesh, we normalise it into unit sphere and choose three angles uniformly from $[0, 2\pi]$ as the value for yaw, pitch, roll: $r_{\{1...9\}}$. The object is centered at the origin of the world frame with zero translations: $t_{\{1,2,3\}}$. Then we use z-buffering to render it into a depth image. The self-occluded point clouds are generated via back-projecting the depth images based on eq.~\ref{eq:world_transform}.
% We choose ModelNet40 as it has a richer class of objects compared to other datasets. 
% Specifically, 
% We sample 10 sets of yaw, pitch and roll uniformly from $[0, 2\pi]$ which yield $\{r_{1}, \ldots, r_9\}$,
% via the standard Euler angle transformation, 
% and set zero translation $t_{\{1,2,3\}}\!=\!0$. 
\textbf{Dataset}: For all experiments, we use ModelNet40~\citep{wu20153d} as the pre-training dataset, a challenging transfer learning setting, as ModelNet40 and fine-tuning datasets may not come from the same domain. ModelNet40 includes 12,311 synthesized objects from 40 categories, divided into 9,843/2,468 objects for training and testing, respectively. We construct a pre-training dataset using the training objects. We generate occluded point clouds with camera intrinsic parameters $\{f=1000, \gamma=0, \omega=1600, h=1200$\}, 10 randomly selected viewpoints and zero translation. Figure~\ref{fig:dataoverview} shows examples of occluded point clouds. 
% Note that these are qualitatively similar to point clouds in datasets where points are collected via 3D imaging devices such as handheld scanners \citep{dai2017scannet,armeni20163d}
% % (ScanNet: \citet{dai2017scannet}, S3DIS, \citet{armeni20163d}) 
% and lidar \citep{KITTI}. 
% (KITTI, \citet{KITTI}). 

% encoders, similar to prior completion models~\citep{Tchapmi_2019_CVPR,WangAL20,WenLHL20}

\textbf{Architecture}: Our pre-training model, a completion model $c(\cdot)$, follows the ``encoder-decoder'' architecture. To validate the generality of our pre-training objective, we choose three different encoders including PointNet~\citep{qi2017pointnet}, PCN~\citep{yuan2018pcn} and DGCNN~\citep{wang2019dynamic}. These encoders encode an occluded point cloud into a 1024-dimensional vector. For decoder, we adapt the folding-based decoder from \citet{yuan2018pcn} to complete an occluded point cloud in two steps. The decoder first output a coarse shape, $\hat{\mathcal{P}}_{coarse}$, with 1024 points then warps a 2D grid around each point in $\hat{\mathcal{P}}_{coarse}$ in order to get a fine shape, $\hat{\mathcal{P}}_{fine}$, which consist of 16384 points. We use Chamfer Distance (CD) as the closeness measure of two point sets:
\begin{gather}
\begin{split}
    \mathrm{CD}(\hat{\mathcal{P}}, \mathcal{P}) = &\frac{1}{|\hat{\mathcal{P}}|}\sum_{\hat{x}\in \hat{\mathcal{P}}}\min_{x\in \mathcal{P}}||\hat{x}-x||_2 \\+ &\frac{1}{|\mathcal{P}|}\sum_{x\in \mathcal{P}}\min_{\hat{x}\in \hat{\mathcal{P}}}||x-\hat{x}||_2.
\end{split}
\end{gather}
The total loss of the completion task is a linear combination of the two Chamfer Distances:
\begin{gather}\label{eq:completion_loss}
    l = \mathrm{CD}(\hat{\mathcal{P}}_{coarse}, \mathcal{P}_{coarse}) + \alpha * \mathrm{CD}(\hat{\mathcal{P}}_{fine}, \mathcal{P}_{fine}),
\end{gather}

% It first generates a sparse set of points to match the overall geometry of the point cloud. Then it generates dense points around the sparse points to approximate a smooth surface. 
% , as we find it performs just as well as the Earth Mover's Distance (EMD), which is slower and must be approximated to run practically~\citet{bertsekas1985distributed}. 
% For further optimization details and a hyperparameter sensitivity study, see the Appendix.
% \paragraph{\abbrev pre-training.}

\textbf{Hyperparameters}: We use Adam~\citep{KingmaB14} as the optimizer. The learning rate is set to 1e-4 initially, and is decayed by 0.7 every 10 epochs. We pre-train the models for 50 epochs. The batch size is 32 and the momentum of batch normalisation is 0.9. The coefficient $\alpha$ in~\eqref{eq:completion_loss} is first set as 0.1 for the first 10000 training steps, then increases to 0.1 and 0.5 at the 20000th and 50000th training steps, respectively. The $\alpha$ is fixed as 1.0 after 50000 training steps. 

\begin{table*}[h!]
\small
\centering
% \vspace{-1ex}
\caption{Comparison between \abbrev, Jigsaw and Rand initialization on 3D object recognition benchmarks.
% , based on PointNet, PCN and DGCNN. 
% Here `*' marks the reported scores from the original literature \citep{qi2017pointnet,wang2019dynamic,ScanObjectNN,sauder2019self} (we additionally confirm these scores are reproducible). 
After confirming the scores from \citep{qi2017pointnet,wang2019dynamic,ScanObjectNN,sauder2019self} are reproducible, we reported the mean and standard deviation over three runs.} % `**' marks our reproduced result which is quite lower than reported in \cite{ScanObjectNN} with the same protocols}
%For the benchmark datasets, the first three, `ShapeNet10', `ModelNet10' and `ModelNet40' are fully synthesized 3D objects based on CAD models, while `ScanNet10' contained the same class as `ShapeNet10' and `ModelNet10' but with occlusion. `ShapeNet Par' and `ModelNet Par' are the data we used for \abbrev tasks, consist of synthesized occluded point clouds, 
% `ScanObjectNN' includes real-world point cloud, which are segmented from entire indoor scans which are occluded, sometime with background noise (bn), we list all the test results on the variations of `ScanObjectNN' in the appendix.
% \vspace{-1ex}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{Dataset} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
% ShapeNet10 & 94.9 & 95.3 & \textcolor{blue}{95.5} & 95.1 & 95.2 & \textcolor{blue}{95.4} & 95.8 & 96.0 & \textbf{96.6} \\\hline
MN40& 89.2$\pm$0.2 & 89.6$\pm$0.2 & \textcolor{blue}{90.1$\pm$0.2} & 89.3$\pm$0.2 & 89.6$\pm$0.3 & \textcolor{blue}{90.3$\pm$0.3} & 92.5$\pm$0.7 & 92.3$\pm$0.5 & \textbf{93.0$\pm$0.3} \\\hline
% ShapeNet Oc & 94.6 & 94.6 & \textcolor{blue}{95.0} & 94.9 & \textbf{95.1} & \textbf{95.1} & 94.5 & 94.4 & \textbf{95.1} \\\hline
% ModelNet Oc & 85.3$\pm$0.2 & 85.5 & \textcolor{blue}{85.6} & 84.6 & \textcolor{blue}{85.1} & \textcolor{blue}{85.1} & 88.7 & 88.7 & \textbf{89.1} \\\hline
ScN10& 76.9$\pm$0.3 & 77.2$\pm$0.3 & \textcolor{blue}{78.0$\pm$0.3} & 77.0$\pm$0.5 & 77.9$\pm$0.5 & \textcolor{blue}{78.2$\pm$0.5} & 76.1$\pm$1.2 & 77.8$\pm$0.9 & \textbf{78.5$\pm$0.5}  \\\hline
SO15 & 73.5$\pm$0.9 & 76.5$\pm$0.7 & \textcolor{blue}{80.0$\pm$0.3} & 78.3$\pm$0.5 & 78.2$\pm$0.2 & \textcolor{blue}{80.4$\pm$0.3} & 82.4$\pm$0.7 & 82.7$\pm$1.4 & \textbf{83.9$\pm$0.7} \\
% ScanObjectNN (OBJ\_ONLY)\cite{ScanObjectNN}& 79.2* & 79.9 & 79.3 & 79.5 & 79.7** & 84.0\\
\toprule
\end{tabular}
\label{tab:classification}
% \vspace{-3ex}
\end{table*}

\subsection{Fine-Tuning Details \label{fine_tuning_details}}
% while Unseen samples are then queried from 
% for testing

% \qi{The contents of this section are a bit cluttered. We can first introduce the four tasks and then introduce the fine-tuning hyperparameters}

\paragraph{Few-shot learning.} Few-shot learning aims to build accurate models with very limited training data, and a common setting is called ``$K$-way $N$-shot''. During training, $K$ classes are randomly selected, and each class contains $N$ samples. The trained model are then evaluated on the objects from the test split. In our experiments, we use ModelNet40 and Syndey10~\citep{de2013unsupervised} for the ``$K$-way $N$-shot'' classification. We use the same setting and train/test split as cTree \citep{sharma2020self}. Each object is represented with 100 points. We use the same training configurations as in the object classification tasks.


%We use the same training settings as used in the next paragraph. 
% The training settings are identical to the ones used in the classification.
% We use the same data and train/test split as \citep{sharma2020self}, the training settings are identical to previous.
% We use the same training settings as our classification experiments, which are identical to the original literature.

\paragraph{Object classification.}
Given an object represented by a set of points, object classification is to predict which class this object belongs to.
We use three 3D object recognition benchmarks: ModelNet40~\cite{wu20153d}, ScanNet10~\citep{pointdan} and ScanObjectNN~\citep{ScanObjectNN}. We summarise the dataset statistics in table~\ref{tab:classification_benchmark}, where the later two are more challenging since they contain the occluded objects from the real indoor scans.
We use the same training settings as the original works. Concretely, for PCN and PointNet, we use the Adam optimizer with an initial learning rate 1e-3, decayed by 0.7 every 20 epochs to a minimum value of 1e-5. For DGCNN, we use the SGD optimizer with a momentum of 0.9 and a weight decay of 1e-4. The learning rate starts from 0.1 and then reduces using cosine annealing~\cite{LoshchilovH17} with a minimum value of 1e-3. We use dropout~\cite{dropout} in the fully connected layers before the softmax output layer. The dropout rate of PointNet and PCN is set to 0.7, and is 0.5 for DGCNN. For all three models, we train them for 200 epochs with a batch size of 32. We report the test results based on three runs in table~\ref{tab:classification}.

\begin{table}[H]
\centering
\small
\vspace{-2ex}
\caption{Statistics of classification datasets}
\begin{tabular}{l|c|c|c|c}
\bottomrule 
Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
MN40& synthesized & 40 & 9,843 & 2,468 \\\hline
% ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
SN10 & real scanned & 10 & 6,110 & 1,769 \\\hline
SO15 & real scanned & 15 & 2,304 & 576 \\
\toprule
\end{tabular}
\label{tab:cls_data}
\vspace{-3ex}
\end{table}

% : ModelNet40, ShapeNet10, ScanNet10, ShapeNet Occluded, ModelNet Occluded and ScanObjectNN (OBJ\_BG). 
% For PointNet and DGCNN baselines, we use the same training settings as the original literature, we adapt the output layers as well as the training setting for PCN based on those of PointNet (in appendix).
% , just as in~\citeps{qi2017pointnet}. 
% : ShapeNet~\cite{chang2015shapenet}, ModelNet40~\cite{wu20153d} and ScanNet10~\cite{pointdan}.
% ShapeNet has more than 3 million CAD models, of which 220,000 models are labeled into 3,135 object categories, making it one of the largest 3D object classification datasets.
% ADD MODELNET
%ShapeNet10 and ScanNet10 are first introduced for domain adaptation~\cite{pointdan}.
% does the below sound okay? this way we don't say we introduce it
% it's a bit confusing to say it was introduced by PCN as they would have to know our model to use our technique, I realize our technique is based on PCN, but I just think it's clearer to say 'we use our occlusion technique' to create both datasets
% hmmm, I see. maybe we can just say in the appendix that we need to improve the quality of that data before using it for pre-training?
% good point
% could we submit the main paper then?
% thanks!
% ohoh, I just want to be consistent with the appendix since the model pre-trained on shapenet occluded mostly performance even worse than random insitilaised ones, that is probably because of the quality of pre-trained data, which is not our responsibility
% okay, this is not the place where the reviewer cares about..
% yead, on it
% ShapeNet10 is sampled from the synthesized dataset ShapeNet~\cite{chang2015shapenet} with 17,378 training examples and 2,492 testing examples. ScanNet10 is derived from scanned and reconstructed real-world indoor scenes~\cite{dai2017scannet} with 6,110  training examples and 1,769 testing examples. We also evaluate on ShapeNet Occluded and ModelNet Occluded, where we use the occlusion mapping described in Section~\ref{subsec:occ} to create occluded point clouds. These datasets are used to evaluate the models on a more challenging scenario where point clouds are partially observable. ModelNet Oc contains 98,430 training CAD models and 24,680 testing models, while ShapeNet Oc consists of 231,792 training examples and 800 testing examples. We also use a real-world scanned indoor scene dataset, ScanObjectNN (OBJ\_BG)~\cite{ScanObjectNN}, which contains 15 categories, 2,304 training objects and 576 testing objects. All point clouds are sub-sampled to 1024 points, just as in~\citet{qi2017pointnet}.
% \begin{table}[H]
% \centering
% \small
% \vspace{-2ex}
% \caption{Statistics of classification datasets}
% \vspace{-2ex}
% \begin{tabular}{l|c|c|c|c}
% \bottomrule 
% Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% % ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
% (MN40) ModelNet40~\citep{wu20153d} & synthesized & 40 & 9,843 & 2,468 \\\hline
% % ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% % ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
% (SN10) ScanNet10~\citep{dai2017scannet} & real scanned & 10 & 6,110 & 1,769 \\\hline
% (SO15) ScanObjectNN ~\citep{ScanObjectNN} & real scanned & 15 & 2,304 & 576 \\
% \toprule
% \end{tabular}
% \label{tab:cls_data}
% \vspace{-3ex}
% \end{table}

\paragraph{Part segmentation.} 
Part segmentation is a challenging fine-grained 3D recognition task. Given a 3D scan, the task is to predict part category label (e.g., chair leg, cup handle) of each point.
We use the ShapeNetPart~\citep{armeni20163d} benchmark for this task, which contains 16,881 objects from 16 categories, and has 50 parts in total.
Each object is represented with 2048 points. We use the same training settings as the original works, for PCN and PointNet, we use the Adam optimizer with an initial learning rate 1e-3, decayed by 0.5 every 20 epochs to a minimum value of 1e-5. For DGCNN, we use the SGD optimizer with a momentum of 0.9 and a weight decay of 1e-4. The learning rate starts from 0.1 and then reduces using cosine annealing~\cite{LoshchilovH17} with a minimum value of 1e-3. For all three models, we train them for 250 epochs with a batch size of 16. We use the same test procedures (majority votes) as the original works, and report the results based on three runs in table~\ref{tab:partseg_result}.


\paragraph{Semantic segmentation.} 
Similar to part segmentation, the point labels in semantic segmentation instead become semantic object classes of an indoor/outdoor scene. We use the S3DIS benchmark~\citep{armeni20163d} for semantic indoor scene segmentation. It contains 3D scans collected via Matterport scanners in 6 different places, encompassing 271 rooms. Each point, described by a 9-dimensional vector (including coordinates, RGB values and normalised location), is labeled as one of 13 semantic categories (e.g. chair, table and floor). We use the same preprocessing procedures and training settings as the original work. 
We also fine tuned and show the effectiveness of our pre-training on a recent urban-scale outdoor point cloud scans~\cite{hu2020towards}. We reported these results in the appendix.

\begin{table}[h!]\small
\centering
% \vspace{-2ex}
\setlength{\tabcolsep}{2pt}
\caption{Few-shot classification results. We report mean and std over 10 runs. We bold the the cell with the largest mean.
% We also bold the cell where its mean + std $>=$ the largest mean.
\label{exp:few_shot_classification} }
\begin{tabular}{l|cccc}
\bottomrule \multicolumn{1}{c|}{\multirow{2}{*}{Baseline}} 
& \multicolumn{2}{c}{5-way} & \multicolumn{2}{c}{10-way} \\ \cline{2-5}
& 10-shot & 20-shot & 10-shot & 20-shot \\ \toprule \bottomrule
3D-GAN & 55.8$\pm$10.7 & 65.8$\pm$9.9 &40.3$\pm$6.5 &48.4$\pm$5.6\\
FoldingNet & 33.4 $\pm$13.1 & 35.8$\pm$18.2 & 18.6$\pm$6.5 & 15.4$\pm$6.8 \\
Latent-GAN & 41.6$\pm$16.9 & 46.2$\pm$19.7 & 32.9$\pm$9.2 & 25.5$\pm$9.9\\
PointCapsNet & 42.3$\pm$17.4 &53.0$\pm$18.7 &38.0$\pm$14.3 & 27.2$\pm$14.9\\
PointNet++ & 38.5$\pm$16.0 & 42.4$\pm$14.2 & 23.1$\pm$7.0 & 18.8$\pm$5.4 \\
PointCNN & {65.4$\pm$8.9} & {68.6$\pm$7.0} & {46.6$\pm$4.8} & {50.0$\pm$7.2} \\
\toprule \bottomrule
PointNet, Rand & 52.0$\pm$12.2 & 57.8$\pm$15.5 & 46.6$\pm$13.5 & 35.2$\pm$15.3 \\
PointNet, cTree & 63.2$\pm$10.7 & 68.9$\pm$9.4 & 49.2$\pm$6.1 & 50.1$\pm$5.0 \\
PointNet, OcCo & \textbf{89.7$\pm$6.1} & \textbf{92.4$\pm$4.9} & \textbf{83.9$\pm$5.6} & \textbf{89.7$\pm$4.6} \\\hline
DGCNN, Rand & 31.6 $\pm$9.0 & 40.8$\pm$14.6 &19.9$\pm$6.5 & 16.9$\pm$4.8\\
DGCNN, cTree & 60.0$\pm$8.9 & 65.7$\pm$8.4 & 48.5$\pm$5.6 & 53.0$\pm$4.1\\
DGCNN, OcCo & \textbf{90.6$\pm$2.8} & \textbf{92.5$\pm$6.0} & \textbf{82.9$\pm$4.1} & \textbf{86.5$\pm$7.1}\\
\toprule
\end{tabular}
% s}
\vspace{-2ex}
\label{tab:fsl}
\end{table}



%\paragraph{Benchmark.} We trained ~\citep{sauder2019self} (Jigsaw) on ModelNet40 and reported in all.
% We compare with~\citep{sharma2020self} in the few-shot settings.
% \textit{\abbrev Pre-training configurations}: 
% %transferability we will only  The dataset for the pretrained completion tasks are based on either ShapeNet \cite{yuan2018pcn} or ModelNet40. %(as we described the construction process in the previous sections). 
% We use the 3D computer graphics software, Blender~\cite{blender}, to generate occluded point clouds. 
% %Then we use eq. \ref{eq:world_transform} to restore the occluded point cloud from the depth images, each pixel in the depth image is correspondent to a spatial point in the occluded point cloud. 
% For the ShapeNet dataset, we consider 
% %we use the data provided by \cite{yuan2018pcn}, which contains
% 30974 objects from 8 categories for pre-training. For each object we generate 8 occluded point clouds from randomly chosen viewpoints. The camera is set to 100, 120 and 160 units for focus, height and width, respectively, of the rendered depth images. The average number of points for each object is around 1000, which is more coarse compared with our pre-processed dataset based on ModelNet40.

% The top half of the table reports results for eight randomly initialized point cloud models, while the bottom-half reports results on two models across three pre-training methods.
\begin{table*}[t!]\small
\centering
\vspace{-1ex}
\caption{Mean point accuracy (mAcc) and intersection of union (mIoU) on ShapeNetPart. We reported the mean and std over three runs.}
% As in Table 2, `*' marks previously reported scores, and \textcolor{blue}{blue} and \textbf{bold} are best scores.
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
mAcc & 92.8$\pm$0.9 & 93.1$\pm$0.5 & \textcolor{blue}{93.4$\pm$0.7} & 92.3$\pm$1.0 & 92.6$\pm$0.9 & \textcolor{blue}{93.0$\pm$0.9} & 92.2$\pm$0.9 & 92.7$\pm$0.9 & \textbf{94.4$\pm$0.7} \\\hline
mIoU & 82.2$\pm$2.4 & 82.2$\pm$2.8 & \textcolor{blue}{83.4$\pm$1.9} & 81.3$\pm$2.6 & 81.2$\pm$2.9 & \textcolor{blue}{82.3$\pm$2.4} & 84.4$\pm$1.2 & 84.3$\pm$1.2 & \textbf{85.0$\pm$1.0} \\
\toprule
\end{tabular}
\vspace{-1ex}
\label{tab:partseg_result}
\end{table*}

\begin{table*}[t!]\small
\centering
\vspace{-1ex}
\caption{Mean point accuracy (mAcc) and class intersection of union (mIoU) on the S3DIS averaged across six folds over three runs.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c|}{PCN} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-10}
 & Rand & Jigsaw & \abbrev& Rand & Jigsaw & \abbrev & Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
mAcc & 78.2$\pm$0.7 & 80.1$\pm$1.2 & \textcolor{blue}{82.0$\pm$1.0} & 82.9$\pm$0.9 & 83.7$\pm$0.7 & \textbf{85.1$\pm$0.5} & 83.7$\pm$0.7 & 84.1$\pm$0.7 & \textcolor{blue}{84.6$\pm$0.5} \\\hline
mIoU & 47.0$\pm$1.4 & 52.6$\pm$1.9 & \textcolor{blue}{54.9$\pm$1.0} & 51.1$\pm$2.4 & 52.2$\pm$1.9 & \textcolor{blue}{53.4$\pm$2.1} & 54.9$\pm$2.1 & 55.6$\pm$1.4 & \textbf{58.0$\pm$1.7}\\
\toprule
\end{tabular}
\label{tab:seg_result}
\end{table*}



\subsection{Fine-Tuning Results \label{fine_tuning_results}}
\subsubsection{Few-Shot Learning \label{sec:fsl}}
The results of few-shot learning are shown in Table \ref{exp:few_shot_classification}. We find that our model outperforms a strong few-shot baseline \cite{sharma2020self}, while both methods can significantly outperform randomly-initialized baselines with different architectures. We therefore conclude that \abbrev can significantly improve the performance of few-shot learning.
\qi{Run few-shot on another dataset in future work}


\subsubsection{Object Classification Results}
\label{sec:classification}
In Table~\ref{tab:classification}, we compare OcCo with random and Jigsaw \citep{sauder2019self} initialization on three object classification datasets with three encoders. ``MN40'', ``ScN10'' and ``SO15'' stand for ModelNet40, ScanNet10 and ScanObjectNN respectively.  We show that OcCo-initialized models outperform the baselines on all the datasets. Especially, OcCo performs well not only on the in-domain dataset (MN40), but also on cross-domain datasets (ScN10 and SO15). The results are consistent across three encoders. These results demonstrate that the representations from \abbrev can transfer to object classification.


\qi{This can be put into the analysis section instead of saying it here: In appendix, we make more comparisons such as training a linear SVM based on the learned features from OcCo pre-training with other autoencoder and GAN based methods.} 

% We compare OcCo-initialized and randomly-initialized models on the object classification datasets. 
% For fine-tuning the downstream models, we use the settings in \cite{qi2017pointnet,wang2019dynamic}, for more details see Appendix~\ref{app:opt}.
 


% , increasing the absolute performance by as much as $33.1\%$ (on ShapeNet10 using the PointNet encoder). 
% The improvements are consistent across all the three encoder networks. 
% We conclude that \abbrev brings architecture-agnostic improvements compared to the random initialization on object classification. 
% \todo{ScanObjectNN(OBJ\_BG)}
%We initialize the weights of the classification model using the \abbrev pre-training weights as follows. We restore the encoder weight from the \abbrev model and then randomly initialize the remaining weights. %for layers with same scopes and shapes, then initialised the rest.
%For randomly initialized models, we initialize all the variables on the same network architecture. 
%We have observed that increasing the number of pre-training epochs does not monotonically improve performance. We discuss this further in Section~\ref{subsec:ss}. %Thus for classification, segmentation and few-shots learning tasks, we use the checkpoints that give the best training performance: 20 epochs with batch size of 64 for the pre-trained PCN-based models, and 10 epochs with batch size of 32 for the pre-trained PointNet-based models. 
%We repeated the training process for 3 times and reported the average in Table~\ref{tab:classification}. 

 %, including ShapeNet10, ScanNet10, ShapeNet Occluded and ScanObjectNN. 
%as well as the random initialised baseline (originally 92.2\%, now updated as 92.9\% in \cite{wang2019dynamic}), which shows the effectiveness of \abbrev compared to \cite{sauder2019self}. 

\subsubsection{Object Part Segmentation Results}
\label{sec:part_seg}
% We now compare \abbrev against prior initialization approaches on object classification tasks. 
% We compare OcCo-initialized and randomly-initialized models on the object classification datasets. 
% For fine-tuning the downstream models, we use the settings in \cite{qi2017pointnet,wang2019dynamic}, for more details see Appendix~\ref{app:opt}.
Table~\ref{tab:partseg_result} compares OcCo-initialization with random and Jigsaw \citep{sauder2019self} initialization on object part segmentation.
% , averaged across 3 trials.
We observe that OcCo-initialized models outperform or perform competitively in accuracy and IoU compared to the other two initializations. The results are consistent across three encoders. This demonstrates that \abbrev can improve object part segmentation, and the improvements are robust to different encoders. %(also in Figure~\ref{fig:tsne}).
% We reported the detailed scores on each individual shape class in the appendix, for total 15 classes, 

\subsubsection{Semantic Segmentation \label{sec:scene_seg}}
Here we compare random, Jigsaw and \abbrev initialization on semantic segmentation. We use $k$-fold cross validation following \citet{armeni20163d}.
% , i.e., split data into $k$-parts and train $k$ models where the test set is one of the $k$ folds and the train set is the remaining $k\!-\!1$ folds. 
%for each hold-out fold, we train a new model based on the examples from the other $k\!-\!1$ folds and test on the hold-out fold). % to produce training and testing sets. 
% During the training, we use a batch size of 24 and training epochs of 50. The learning rate is set as 1e-3 initially, decayed to half for every 300,000 iterations and then is clipped to ensure it does not drop below 1e-5.
The results are reported in Table \ref{tab:seg_result}. OcCo-initialized models outperform random and jigsaw-initialized ones, demonstrating that \abbrev pre-training can bring in significant improvements for semantic segmentation.\footnote{We notice that the best model in \citet{sauder2019self} (mIoU=41.2) underperforms the result in DGCNN~\cite{wang2019dynamic} (mIoU=56.1). They consider a transductive setting which is not directly comparable to ours, so here we stick to the supervised setting and report our reproduced scores. \qi{Cannot understand this sentence.}}

\section{Analysis}\label{subsec:probe-test}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{resources/PT.pdf}
    \caption{Visualisation on the learned features by OcCo-pretrained PointNet.}
    \label{fig:tsne}
\vspace{-1ex}
\end{figure*}
In this section, we perform extensive analyses to study the reasons for OcCo's success. We first show that \abbrev can improve sample efficiency and convergence in downstream tasks. Then, we use three techniques, including semantic concept detection, unsupervised mutual information probe and visualization, to demonstrate that a model pre-trained with \abbrev can extract rich and discriminative point cloud features even without fine-tuning. 

%  Since point cloud encoders usually learn each point feature either independently or via neighborhood aggregation, the feature maps usually do not change in the vertical direction (see Figure~\ref{fig:tsne}). Therefore we can skip the \emph{retrieval} step and directly quantify the alignment between
\qi{Why use ModelNet for sample efficiency experiment? The setting is a bit weird. This assumes that the downsteam task is in the same domain as the pre-training data. todo: test on another dataset, e.g. Shapenet for sample efficiency. Then report the results on both modelnet and another dataset for sample efficiency. The results on Pointnet do not seem very well. Maybe remove that part.}
\paragraph{Sample Efficiency.} We investigate whether \abbrev pre-training can improve sample efficiency in downstream tasks. To this end, we randomly select 1\%, 5\%, 10\% and 20\% of samples from training set for fine-tuning. The fine-tuned models are evaluated on full test set. As shown in Table \ref{tab:few_shot}, models with \abbrev pre-training achieve better results compared to models with either random or Jigsaw initialization, which confirms the effectiveness of OcCo pre-training for boosting sample efficiency. 

\qi{The ModelNet figures are from the sample efficiency experiments, which is a bit weird compared to the others, e.g. S3DIS, which is full set}
\paragraph{Convergence.} We study the effect of pre-training on convergence in downstream tasks. We plot learning curves during fine-tuning. The results for classification (ModelNet and ScanObjectNN) and segmentation (S3DIS) are shown in Figure~\ref{fig:learning_curves}. We observe that the models with \abbrev initialization converge faster and better than the models with random or  Jigsaw initialization. This shows that \abbrev pre-training can improve convergence in downstream tasks.

% For ScanObjectNN with DGCNN encoder, the OcCo-initialized model converges around 20 epochs and to a better test accuracy than the random and Jigsaw-initialized model. 
\begin{table}[t!]\small
\centering
\setlength{\tabcolsep}{4pt}
\caption{Sample efficiency with randomly, Jigsaw and OcCo-initialized models on ModelNet40. We use 1\%, 5\%, 10\% and 20\% of the training data and evaluate the model on the full test set.} %\abbrev initialization uses models pre-trained on the occluded dataset from ModelNet40.}
\begin{tabular}{c|c|c|c|c|c|c}
\bottomrule \multirow{2}{*}{Baseline} & 
\multicolumn{3}{c|}{PointNet} & \multicolumn{3}{c}{DGCNN} \\ \cline{2-7}
 & Rand & Jigsaw & \abbrev&  Rand & Jigsaw & \abbrev \\ \toprule \bottomrule
1\%  & 56.9 & 55.7 & \textcolor{blue}{58.1} & 60.0 & 59.9 & \textbf{60.5} \\\hline
5\%  & 73.9 & 74.3 & \textcolor{blue}{74.9} & 79.4 & 79.2 & \textbf{79.7} \\\hline
10\% & 80.6 & \textcolor{blue}{81.3} & 81.1 & 84.4 & 84.4 & \textbf{84.5} \\\hline
20\% & 83.6 & \textcolor{blue}{84.2} & \textcolor{blue}{84.2} & 86.5 & 86.7 & \textbf{87.2} \\ %\hline %\hline
\toprule
\end{tabular}
\vspace{-3ex}
\label{tab:few_shot}
\end{table}
\begin{figure}[h!]
    \centering
     \includegraphics[width=0.5\textwidth]{resources/learning_curve_short.pdf}
     \vspace{-3ex}
     \caption{Learning curves of random, Jigsaw and OcCo-initialised models on fine tuning tasks.}
     \label{fig:learning_curves}
     \vspace{-1ex}
\end{figure}

\paragraph{Detection of semantic concepts.} We adopt \emph{network dissection}~\citep{bau2017network,bau2020understanding} to study whether \abbrev-pretrained models without fine-tuning can learn semantic concepts in an unsupervised fashion. Specifically, for each point cloud, network dissection first creates a binary mask $M_k$ based on the feature map from the $k$-th channel. If the activation of a point in the feature map is larger than a threshold, its mask value is 1. Otherwise its mask value is 0. $M_k$ is compared with the $n$-th concept mask $C_n$, which comes from ground-truth segmentation labels, e.g.\ the concept mask value is 1 if it belongs to an object part like the leg of a chair. Given a set of point clouds $\mathcal{D}_\mathcal{P}$, these masks are used to calculate the mean intersection of union (mIoU):
\begin{gather}
    \text{mIoU}_{(k, n)}=
    \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}
    \left[\frac{\left|M_{k}(\mathcal{P}) \cap C_{n}(\mathcal{P})\right|}
    {\left|M_{k}(\mathcal{P}) \cup C_{n}(\mathcal{P})\right|}\right]
\end{gather}
where  $|\cdot|$ is the set cardinality. Network dissection calculates the expectation of the intersection of the two masks divided by the union of the two masks. $\text{mIoU}_{(k, n)}$ can be interpreted as how well channel $k$ detects the concept $n$. In Figure~\ref{fig:feat-det}, we plot the number of concepts detected by either Jigsaw or \abbrev. \abbrev outperforms Jigsaw in terms of the total number of detected concepts. This demonstrates that pre-training with \abbrev can unsupervisedly learn semantic concepts.

\begin{figure}
    \centering
     \includegraphics[width=0.45\textwidth]{resources/learned_feat_short.pdf}
     \vspace{-3ex}
     \caption{Visualisation of detected concepts (e.g., chair backs, car wheels and headset bands) from the OcCo-initialised PointNet. Parts marked by blue are based on the generated binary mask from the specified unit, the green ones are annotated as the ground truth. \qi{Put this visualization to corresponding sections}}
    %  \label{fig:learning_curves}
     \vspace{-1ex}
\end{figure}

\begin{table*}[h]\small
\centering
\vspace{-1ex}
\caption{Adjusted mutual information (AMI) under transformations. We reported the mean and standard deviation over 10 random initialisation. Under the `transformation' column, `J', `T', `R' represent jittering, translation and rotation respectively.}
% \vspace{-2ex}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\bottomrule \multicolumn{3}{c|}{Transformation} & \multicolumn{4}{c|}{ShapeNet10} & \multicolumn{4}{c}{ScanObjectNN} \\ \hline
J & T & R & VFH & M2DP & Jigsaw & \abbrev & VFH & M2DP & Jigsaw & \abbrev \\ \toprule \bottomrule
& & & 0.12$\pm$0.01 & 0.22$\pm$0.03 & 0.33$\pm$0.04 & \textbf{0.51$\pm$0.03} & 0.05$\pm$0.02 & 0.18$\pm$0.02 & 0.29$\pm$0.02 & \textbf{0.44$\pm$0.03} \\\hline
\checkmark & & & 0.12$\pm$0.02 & 0.19$\pm$0.02 & 0.32$\pm$0.02 & \textbf{0.45$\pm$0.02} & 0.06$\pm$0.02 & 0.17$\pm$0.02 & 0.27$\pm$0.02 & \textbf{0.42$\pm$0.04} \\\hline
\checkmark & \checkmark & & 0.13$\pm$0.03 & 0.21$\pm$0.02 & 0.29$\pm$0.07 & \textbf{0.38$\pm$0.04} & 0.04$\pm$0.02 & 0.18$\pm$0.03 & 0.24$\pm$0.04 & \textbf{0.39$\pm$0.06} \\\hline
\checkmark & \checkmark & \checkmark & 0.07$\pm$0.03 & 0.20$\pm$0.04 & 0.28$\pm$0.03 & \textbf{0.35$\pm$0.05} & 0.04$\pm$0.01 & 0.16$\pm$0.03 & 0.18$\pm$0.09 & \textbf{0.34$\pm$0.06} \\\hline
\toprule
\end{tabular}
\label{tab:so3}
\end{table*}
\vspace{3ex}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=1\textwidth]{resources/Feat_Det_Full.pdf}
    % \includegraphics[width=1\textwidth]{resources/Feat_Det_Short.pdf}
    \vspace{-3ex}
    \caption{Number of (unique) detected object parts in the `Feat1'~(above), `Feat2'~(middle) and `Feat3'~(below) module of Jigsaw and OcCo-initialised PointNet feature encoder. Digits in the bracket are the number of parts in that object category.}
    \label{fig:feat-det}
\end{figure*}

\paragraph{Unsupervised mutual information probe.} We hypothesize that a pre-trained model without fine-tuning can learn label information in an unsupervised fashion. For validation, we take PointNet pretrained with ModelNet40 to extract features for ShapeNet10 and ScanObjectNN. Then, we cluster the features with an unsupervised clustering method, K-means (where K is set to the number of ground-truth labels). To evaluate the quality of clustering, we calculate the adjusted mutual information (AMI)~\citep{nguyen2009information} between the predicted clusters and the ground-truth clusters obtained with class labels. AMI is 1 if these two clusterings are identical, while it has an expected value of 0 for a random clustering. Besides, we also study whether the pre-trained PointNet is robust to input transformations. In particular, we consider three transformations, including rotation, translation and jittering. Therefore, we apply these transformations to an input point cloud, before using PointNet to extract its features for clustering. 

We compare Jigsaw, \abbrev and two hand-crafted point cloud global descriptors: viewpoint feature histogram (VFH)~\citep{rusu2010fast} and M2DP~\citep{he2016m2dp} in Table~\ref{tab:so3}. We observe that pre-training methods, e.g.\ Jigsaw and \abbrev, can learn more discriminative feature representations compared to handcrafted descriptors, while the representations from \abbrev are more predictive than Jigsaw. These results demonstrate that \abbrev is an effective approach for unsupervised feature learning.

%We show that \abbrev pre-training helps the networks to learn better embeddings of point cloud objects, especially when they are occluded and with outlier points (ScanObjectNN).


%We use  based on the clustering $\Omega$ and the ground truth label $\mathcal{C}$, 


% Based on normalised mutual information (NMI), 
%Therefore it allows direct comparisons between different datasets:
%\begin{gather}
%    \mathrm{AMI}(\Omega, \mathcal{C}) = 
%    \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}
%    \left[\frac{\mathrm{I}(\Omega; \mathcal{C})- \mathbb{E}[\mathrm{I}(\Omega; \mathcal{C})]}{(\mathrm{H}(\Omega)+\mathrm{H}(\mathcal{C}))/2- \mathbb{E}[\mathrm{I}(\Omega;\mathcal{C})]}\right]
%\end{gather}
%where $\Omega$ is the clustering determined by the learned embeddings $\mathrm{Enc}(\cdot)$ and unsupervised clustering methods such as K-means. $\mathrm{I}(\Omega ; C)=\sum_{k} \sum_{j} P\left(w_{k} \cap c_{j}\right) \log \frac{P\left(w_{k} \cap c_{j}\right)}{P\left(w_{k}\right) P\left(c_{j}\right)}$ denotes the mutual information, $\mathrm{H}(\cdot)$ is the entropy. 

%It is calculated as:
%\begin{gather}
%    \mathcal{L} = \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P},\mathcal{S}\sim \mathrm{SO(3)}}\left[\operatorname{AMI}(\Omega, \mathrm{Enc}(\mathcal{S}(\mathcal{P})))\right]
%\end{gather}





% $\text{mIoU}_{(k, n)}=\mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}(\mathrm{IoU}(M_{k}(\mathcal{P}), C_{n}(\mathcal{P}))) > 0.5$. 
% For random and pre-trained encoders, we counts the number of detectors over all features and concepts. 

% For NMI, we compare the performance of the clustering methods based on i) coordinates ii) coordinates + learned features.

% The calculation of the expectation $ \mathbb{E}[\mathrm{I}(\mathcal{C}; \mathcal{C}')]$ is provided in ~\citep{nguyen2009information}. 
%AMI has a maximal of 1 when two partitions are identical, and reaches a minimal of 0 if two clusters are total uncorrelated. 
% \paragraph{Invariance/Equivariance under SO(3) transformation}
% Similar with previous work~\citep{deng2018ppf}, we want the learned embeddings to be invariant or equivariant under rigid SO(3) transformations (i.e., rotation, translation, permutation). 

% where $d(\cdot, \cdot)$ is a distance metric such as $l2$ or cosine,  $\mathrm{Enc}(\cdot)$ is the pre-trained point cloud encoder. 
% Although single representation might vary after SO(3), we want the cluster structures to be preserved.
% We build up the partial point cloud datasets from either ShapeNet or ModelNet. The existed ShapeNet one is used by PCN and TopNet, and the ModelNet is created by ourselves with various resolutions which provide a coarse-to-fine scale for pretraining.
% Once we learn pre-trained \abbrev weights on the ModelNet40, we will demonstrate the encoder weights improve initialization over prior baselines for downstream tasks: object classification, object part and scene semantic segmentation, \emph{on any dataset}. This setup is challenging as the pre-training domain can be very different from the downstream domains. We detail the downstream tasks below.
%\paragraph{Probe test.} 


% For ModelNet40, we generate 10 occluded point clouds for each object from random viewpoints. 
% In order to assess representation transferability, we also use the ModelNet40 pre-training mechanism for training ScanNet10 models. Besides, we perform a more rigorous test of the transferability of pre-training datasets in Section 4.4).
%In order to test transferability of representations we do not 
%The camera's focus and rendered image width and height are 10 times that of the PCN, which provides the pretrained model a board and fine structured of 3D objects, and in section 4.4, we have shown that our dataset are better for the pretraining in terms of the performance of downstream tasks.



% \begin{table}[H]
% \centering
% \small
% \vspace{-2ex}
% \caption{Statistics of classification datasets}
% \vspace{-2ex}
% \begin{tabular}{l|c|c|c|c}
% \bottomrule 
% Name & Type & \# Class & \# Training & \# Testing  \\\toprule \bottomrule
% ShapeNet10~\citep{chang2015shapenet} & synthesized & 10 & 17,378 & 2,492 \\\hline
% ModelNet40~\citep{wu20153d} & synthesized & 40 & 9,843 & 2,468 \\\hline
% ShapeNet Oc~\citep{yuan2018pcn}  & synthesized & 8 & 231,792 & 800 \\\hline
% ModelNet Oc (Our pre-training) & synthesized & 40 & 98,430 & 24,680 \\\hline
% ScanNet10~\citep{dai2017scannet} & real scanned & 10 & 6,110 & 1,769 \\\hline
% ScanObjectNN ~\citep{ScanObjectNN} & real scanned & 15 & 2,304 & 576 \\
% \toprule
% \end{tabular}
% \label{tab:so3}
% \vspace{-3ex}
% \end{table}

\paragraph{Visualisation of learned features.} We use visualization to explore what a pre-trained model without fine-tuning learn about point cloud features. In Figure~\ref{fig:tsne}, we visualize the features of the objects from test split of ModelNet40~\citep{46832}. We color the points according to their channel activations. If the activation is large, its color is dark. Otherwise the color is light. We find that, the pre-trained encoder is able to learn low-level geometric primitives, e.g., planes, cylinders and cones, in the early stage while the network recognises more complex shapes like wings, leafs and upper bodies. We further use t-SNE to visualize the features on ShapeNet10. We notice that distinguishable clusters are formed after pre-training. We therefore conclude that \abbrev can learn features that are useful to distinguish different parts of an object or a scene. These features will be beneficial to downstream tasks, e.g.\ object recognition and scene segmentation.

%is widely used to qualitatively understand the role of a convolutional neural network unit. It links highly activated parts of a CNN channel with human concepts which have semantic meaning. 

% We call channel $k$ a detector of concept $n$ when $\text{mIoU}_{(k, n)}$ is larger than a threshold value.

% \paragraph{Clustering on learned features for part segmentation}
% We can further analyse how helpful the learned features are
% % convex decompositions 
% on distinguishing semantic parts.
% % by comparing ACD with human part annotations on 400 shapes from ShapeNetPart, 
% We use clustering methods including K-means, spectral clustering and hierarchical agglomerative clustering (HAC) based on the coordinates of point clouds $\mathcal{P}_c$ fused w/wo learned features $\mathcal{F}_k$.
% % and approximate convex decompositions (ACD) based on the geometry of the point clouds $\mathcal{P}$.
% We set the number of clusters $N$ to be the amount of annotated parts in each shape $\mathcal{P}$. Given the set of $M$ parts $\mathcal{W}=\left\{w_{1}, w_{2}, \ldots w_{M}\right\}$ and the set of $N$ clusters $\mathcal{C}=\left\{c_{1}, c_{2}, \ldots c_{N}\right\}$, improved clustering performance is evaluated using differences in the normalized mutual information (NMI):
% \begin{gather}
%     \mathrm{NMI}(\mathcal{W}, \mathcal{C}) = \mathbb{E}_{\mathcal{P}\sim\mathcal{D}_\mathcal{P}}\left[\frac{\mathrm{I}(\mathcal{W}; \mathcal{C})}{(\mathrm{H}(\mathcal{W}) +  \mathrm{H}(\mathcal{C}))/2}\right]
% \end{gather}
% where $\mathrm{I}(\mathcal{W}; \mathcal{C})=\sum_{i=1}^{|\mathcal{W}|} \sum_{j=1}^{|\mathcal{C}|} P(w_i, c_j) \log \left(\frac{P(w_i, c_j)}{P(w_i) P(c_j)}\right)$ denotes the mutual information between classes $\mathcal{W}$ and clusters $C$, and $\mathrm{H}(\cdot)$ is the entropy. Better clusterings result in higher NMIs ($\in$ [0,1]).

% \paragraph{Clustering on learned embeddings for classification}


% \subsection{Learning Curves}
% \label{subsec:train_convergence}
% We plot the learning curves for classification and segmentation tasks in Figure~\ref{fig:learning_curves}. We observe that the models with \abbrev initialization converge faster to better test accuracy than the random and sometimes Jigsaw-initialized models. For example, on ModelNet40 with a PCN encoder, the OcCo-initialized model takes around 10 epochs to converge, while the randomly initialized model takes around 50 epochs. Similarly, for %S3DIS with PointNet encoder and 
% ScanObjectNN with DGCNN encoder, the OcCo-initialized model converges around 20 epochs and to a better test accuracy than the random and Jigsaw-initialized model. % large performance gains. 
%We conclude that \abbrev can 
%improve generalization and achieve better or comparable convergence speed on downstream tasks. 


==> sections/introduction.tex <==

Point clouds are a natural representation of 3D objects. 
% They are crucial for various real-world applications in robotics~\citep{yan2019data}, autonomous driving~\citep{li20173d, yue2018lidar}, and localization~\citep{elbaz20173d,angelina2018pointnetvlad}.
Recently, there has been a flurry of exciting new point cloud models in areas such as 
% semantic and instance 
segmentation~\citep{landrieu2018large,yang2019learning,hu2019randla} and object detection~\citep{zhou2018voxelnet,lang2019pointpillars,wang2020pillar}.
% , and scene reconstruction~\citep{li2016manhattan}. 
Current 3D sensing modalities (\textit{i.e.}, 3D scanners, stereo cameras, lidars) have enabled the creation of large repositories of point cloud data~\citep{Rusu_ICRA2011_PCL,hackel2017isprs}. However, annotating~point clouds is challenging as: (1) Point cloud data can be sparse and at low resolutions, making the identity of points ambiguous; (2) Datasets that are not sparse can easily reach hundreds of millions of points (e.g., small dense point clouds for object classification~\citep{zhou2013complete} and large vast point clouds for 3D reconstruction \citep{zolanvari2019dublincity});
(3) Labelling individual points or drawing 3D bounding boxes are both more complex and time-consuming compared with annotating 2D images~\citep{wang2019latte}.
Since most 
% deep learning 
methods require dense supervision, the lack of annotated point cloud data impedes the development of novel models.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{resources/occo2.pdf}
    \vspace{-3ex}
    % \caption{\method\, is a self-supervised pre-training method composed of two steps: (a) occlusion $o(\cdot)$ of an input point cloud $\mathcal{P}$ based on a random camera view-point into a partial point cloud $\tilde{\mathcal{P}}$, and (b) a model $c(\cdot)$ that completes the occluded point cloud $\bar{\mathcal{P}}$ so that $\bar{\mathcal{P}} \approx \mathcal{P}$. We demonstrate that the completion model $c(\cdot)$ can be used as initialization for downstream tasks (e.g., classification, segmentation) leading to faster training and better generalization over existing methods.}
    \caption{A simple method for point cloud pre-training: 1. Take any point cloud dataset and generate occluded point clouds for each input by  (a) randomly sampling a camera view-point, and (b) removing any points hidden from that view-point (for all experiments \emph{we use the same occluded dataset generated from ModelNet40}); 2. Train an encoder-decoder model to complete the occluded point clouds (the encoder can be any model that learns representations of point clouds, the decoder can be any completion model); 3. Use the learned encoder weights as initialization for any point cloud task (e.g., few-shot learning, object classification, part segmentation, semantic segmentation). Surprisingly, this method outperforms a variety of pre-training methods across multiple models and tasks.}
    %\caption{\abbrev  consists of two steps: (a) occlusion $o(\cdot)$ of a point cloud $\mathcal{P}$ based on a random camera view-point into a partial point cloud $\tilde{\mathcal{P}}$, and (b) a model $c(\cdot)$ that completes the occluded point cloud $\bar{\mathcal{P}}$ so that $\bar{\mathcal{P}} \approx \mathcal{P}$. We demonstrate that the completion model $c(\cdot)$ can be used as initialization for downstream tasks, leading to faster training and better generalization over existing methods.}
    \label{fig:overview}
    \vspace{-3ex}
\end{figure}


On the other hand, because of the rapid development of 3D sensors, unlabelled point cloud datasets are abundant. Recent work has developed unsupervised pre-training methods to learn initialization for point cloud models. 
These are based on designing novel generative adversarial networks (GANs)~\citep{wu2016learning,han2019view,achlioptas2017learning} and autoencoders~\citep{hassani2019unsupervised,li2018so,yang2018foldingnet}. However, completely unsupervised pre-training methods have been recently outperformed by the self-supervised pre-training techniques of \citep{sauder2019self} and \citep{alliegro2020joint}. Both methods work by first voxelizing point clouds, then splitting each axis into $k$ parts, yielding $k^3$ voxels. Then, voxels are randomly permuted, and a model is trained to rearrange the permuted voxels back to their original positions. The intuition is that such a model learns the spatial configuration of objects and scenes. 
However, such random permutation destroys all spatial information that the model could have used to predict the final object point cloud. 
% This potentially leads to prediction ambiguities: if two different objects have the same number of point cloud coordinates, then their random permutations are indistinguishable from each other. 

Our insight is that partial point-cloud masking is a good candidate for pre-training in point-clouds because of two reasons: (1) The pre-trained model requires spatial and semantic understanding of the input point clouds to be able to reconstruct masked shapes. (2) Mask-based completion tasks have become the \textit{de facto} standard for learning pre-trained representations in natural language processing (NLP) \citep{mikolov2013efficient,devlin2018bert,peters2018deep}. 
%been proven to be effective in learning pre-trained representations for language data. 
%This poses a number of practical limitations on learning. 1. Manual labeling of point cloud datasets for standard supervised learning problems is nearly always impractical (indeed annotating such datasets warrants a paper in its own right \cite{zolanvari2019dublincity}); 2. Models need to be carefully designed to allow for efficient training over such large datasets. Even models that have linear computation complexity in the dataset size must have small constant factors (e.g., few training epochs).
%and computer vision (CV) \cite{he2019momentum,chen2020simple} communities, %yet studies of self-supervised learning for point clouds are scarce, 
%we propose a novel pre-training mechanism, inspired by masked language modelling \cite{devlin2018bert}. % and shape completion \cite{yuan2018pcn} in CV. 
Different from random permutations, masking respects the spatial constraints that are naturally encoded in point clouds of real-world objects and scenes. Given this insight, we propose \emph{\method} (OcCo) a self-supervised pre-training method that consists of (a) a mechanism to generate occluded point clouds, and (b) a completion task to reconstruct the occluded point clouds. 

Specifically, in (a) point clouds are generated by determining what part of objects would be occluded if the underlying object was observed from a particular view-point. In fact, many point clouds generated from a fixed 3D sensor will have occlusions exactly like this. 
%The intuition is that point clouds collected in real-world will be like this.
% likely be in this way. 
Given an occluded point cloud, the goal of the completion task (b) is to learn a model that accurately reconstructs the missing parts of the point cloud. %The idea is that in order 
For a model to perform this task well, it needs to learn to encode localized structural information, based on the context and geometry of partial objects. % of a partial point cloud. 
This is something that is useful for any point cloud model to know, even if used only for classification or segmentation. 
%that is required to complete
%occlude portions of the point cloud, and learn a representation that can be used to accurately recreate the missing occluded points. Specifically, we generate occluded point-clouds by determining what points would be obstructed if the underlying object was observed from a particular view-point. 

We demonstrate that the weights learned by our pre-training method \emph{on a single unsupervised dataset} can be used as initialization for models in downstream tasks (e.g., object classification, part and semantic segmentation) to improve them, \emph{even on completely different datasets}. Specifically our pre-training technique:
%to improve generalization for object classification
%can obtain problem and domain-independent representations of point clouds. These representations have the following benefits:
%\begin{itemize}[leftmargin=*]
(i) leads to improved generalization over prior baselines on the downstream tasks of object classification, object part and scene semantic segmentation;  
(ii) speeds up 
%It transfers to different datasets: pre-training on one dataset improves task accuracy on others.
model convergence, in some cases, by up to $5\times$; 
(iii) maintains improvements as the size of the labelled downstream dataset decreases; 
(iv) can be used for a variety of state-of-the-art point cloud models.
% \footnote{Our code will be released upon acceptance.}

%\end{itemize}
% (a) improve generalization on downstream tasks, 
% (b) transfer to different datasets, 
% (c) reduce training time, even up to $5\times$, and 
% (d) are more effective than previous pre-training methods.

% We begin by reviewing major related work,
% on deep models for point clouds and pre-training techniques
% then detail our approach and show how it achieves state-of-the-art results in a fraction of typical training time.
% HERE
%only improve generalization on downstream tasks including classification and semantic segmentation, even on different datasets, but also speed up training.
%We propose an alternative self-supervised pre-training mechanism for point cloud models that we demonstrate addresses the lack of label information, improving generalization, and 
%HERE
%We demonstrate that by learning to reconstruct these partial point clouds, our model outperforms all other point-cloud initializations: improving generalization accuracy, and reducing training time for state-of-the-art models in some cases by an order of magnitude.

%     \2 Recent work that has attempted to learn improved initializations either:
%         \3 Can only be used in restrictive settings (GANs)
%         \3 Learn uninformed low-dimensional representations
%         \3 Destroy important spatial information
%To tackle the first problem, 


==> sections/method.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{resources/data_overview_new.pdf}
    \vspace{-2ex}
    \caption{Examples of generated self-occluded objects.}
    \label{fig:dataoverview}
\end{figure*}
We now introduce \method\,(OcCo). Our approach is shown in Figure~\ref{fig:overview}. Our main insight is that by continually occluding point clouds and learning a model $c(\cdot)$ to complete them, the weights of the completion model can be used as initialization for downstream tasks (e.g., classification, segmentation)
, speeding up training and improving generalization over other initialization techniques.
%procedures include two steps: occlusion, then completion. Occlusion is realized by rendering methods and completion is via deep learning based methods.


Throughout we assume point clouds $\mathcal{P}$ are sets of points in 3D Euclidean space, $\mathcal{P} = \{ p_1, p_2, ..., p_n \}$, where each point $p_i$ is a vector of coordinates $(x_i, y_i, z_i)$ and features (e.g. color and normal). 
We begin by describing the components that make up our occlusion mapping $o(\cdot)$. 
Then we detail how to learn a completion model $c(\cdot)$, giving pseudocode and the architectural details in appendix.
Finally we discuss the criteria on validating the effectiveness of a pre-training model for 3D point clouds.
% how helpful OcCo is  for various downstream tasks. 
% what we want from a pre-training tasks.
%We begin with an overview of the approach. We then review pinhole camera basics and how to specify view-points. We give our procedure for masking. We detail and give pseudocode for the completion task. Finally we give technical details we use to implement our approach.

%\subsection{Overview}
 
\subsection{Generating Occlusions}
\label{subsec:occ}
We first describe a randomized occlusion mapping $o: \mathbb{P} \rightarrow \mathbb{P}$ (where $\mathbb{P}$ is the space of all point clouds) from a full point cloud $\mathcal{P}$ to an occluded point cloud $\tilde{\mathcal{P}}$. %\footnote{Where $\mathbb{P}$ is the space of all point clouds.} 
We will do so by determining which points are occluded when the point cloud is viewed from a particular camera position. This requires three steps: 
(1) A projection of the point cloud (in a world reference frame) into the coordinates of a camera reference frame;
(2) Determining which points are occluded based on the camera view-points;
(3) Mapping the points back from the camera reference frame to the world reference frame. 
%We describe each of these in detail.

\paragraph{Viewing the point cloud from a camera.}
A camera defines a projection from a 3D world reference frame into a distinctive 3D camera reference frame. 
It does so by specifying a camera model and a camera view-point from which the projection occurs. 
The simplest camera model is the pinhole camera, and view-point projection for it 
% \footnote{In our experiments we will use a more sophisticated lens camera model. However, any camera model can be used. Thus, to avoid unnecessarily complicating the approach, we describe it in terms of the pinhole camera.}. 
%the projection for the pinhole camera 
is given by a simple linear equation:
%Specifically, this projection can be divided into two parts (a) a perspective projection into camera coordinate space, (b) a normalization by the third dimension. Part (a) is a linear projection that can be written as follows:
\begin{align}
    \begin{bmatrix}
    x_{\text{cam}} \\
    y_{\text{cam}} \\
    z_{\text{cam}} \\
    \end{bmatrix} = 
    \underbrace{\vphantom{
            \left[
                \begin{array}{ccc|c}
                r_1 & r_2 & r_3 & t_1 \\
                r_4 & r_5 & r_6 & t_2 \\
                r_7 & r_8 & r_9 & t_3
                \end{array}
            \right]}
        \begin{bmatrix}
        f & \gamma & w/2 \\
        0 & f      & h/2 \\
        0 & 0      & 1
        \end{bmatrix}}_{
            \substack{\text{intrinsic} \\ [ \;\;\;\; \mathbf{K} \;\;\;\; ]}}
    \underbrace{
        \left[
        \begin{array}{ccc|c}
        r_1 & r_2 & r_3 & t_1 \\
        r_4 & r_5 & r_6 & t_2 \\
        r_7 & r_8 & r_9 & t_3
        \end{array}
        \right]
    }_{\subalign{\text{rotation } &| \text{ translation} \\ [\;\;\;\mathbf{R}\;\;\;\;\; &| \;\;\;\;\;\;\;\mathbf{t}\;\;\;\;\;]}}
    \begin{bmatrix}
    x \\
    y \\
    z \\
    1 
    \end{bmatrix}.
    \label{eq:camera_transform}
\end{align}
In the above, $(x,y,z)$ are the original point cloud coordinates, the matrix including $r$ and $t$ entries is the concatenation of a 3D rotation matrix with a 3D translation vector, and the final matrix to the left is the camera intrinsic matrix ($f$ specifies the camera focal length, $\gamma$ is the skewness between the $x$ and $y$ axes in the camera, and $w,h$ are the width and height of the camera image). Given these, the final coordinates $(x_{\text{cam}},y_{\text{cam}},z_{\text{cam}})$ are the positions of the point in the camera reference frame. We will refer to the intrinsic matrix as $\mathbf{K}$ and the rotation/translation matrix as $[\mathbf{R} | \mathbf{t}]$.

%Part (b) is easily done by dividing $x_{\text{cam}},y_{\text{cam}}$ by $z_{\text{cam}}$. However, if we skip part (b) 


\paragraph{Determining occluded points.}
We can think of the point $(x_{\text{cam}},y_{\text{cam}},z_{\text{cam}})$ in multiple ways: (a) a 3D point in the camera reference frame; (b) a 2D pixel with coordinates $(f x_{\text{cam}}/z_{\text{cam}}, f y_{\text{cam}}/z_{\text{cam}})$ with a depth of $z_{\text{cam}}$. In this way, some 2D points resulting from the projection may be occluded by others if they have the same pixel coordinates, but appear at a larger depth. To determine which points are occluded, we first use \emph{Delaunay triangulation} to reconstruct a polygon mesh from the points, and remove the points which belong to the hidden surfaces that are determined via \emph{z-buffering}.

% However, because point clouds only sparsely cover object surfaces, we need a way to (i) approximate the surface of the point cloud, and then (ii) determine which points are hidden by these surfaces. To approximate the surface (i) we create a polygon mesh of the camera reference point cloud (e.g., via Delaunay triangulation). Solving (ii) is referred to in computer graphics as the problem of \emph{hidden-surface determination}.
% To solve this problem we use a well-known, highly-optimized technique called \emph{z-buffering}. Z-buffering, also referred to as depth-buffering, works by continually estimating the minimum depth of each image pixel in the camera reference frame. It starts with an initial depth buffer of infinite distance for each pixel. Then by looping over each polygon faces of the 3D object, and each pixel in each polygon, z-buffering checks if the depth of that pixel is less than the depth in the buffer. If it is, it updates the depth buffer with the smaller depth. Thus, cloud points at a certain pixel are occluded if all surrounding polygons are at depths greater than the depth of that pixel in the final depth buffer. We remove all these occluded cloud points.  %Z-buffering resolves overlap problems encountered in Painter's algorithm because it considers depth on a per-pixel basis in an order invariant way. 
%In practice, we use the efficient \emph{Blender} package to create meshes and perform z-buffering. 
%render the depth images based on the polygon mesh forms of objects in ModelNet40\cite{wu20153d}, which we will discuss more in Section~\ref{subsec:OcCo-Tech}.


%We briefly review ray tracing, the method we will use to define our randomized occlusion mapping $o(\cdot)$.
%\subsection{Masking via Self-Occlusion}
%\label{Subsec:masking}
%We describe a few representative methods for solving this problem, and how we will use them to construct our randomized mapping $o(\cdot)$.

% \paragraph{Painter's algorithm.}
% Arguably the simplest approach is Painter's algorithm. The idea is based on how a painter might draw a set of objects that overlap each other. Starting with the farthest objects, an artist draws objects that are increasingly closer, allowing the closer objects to overlap the farther ones. More specifically, the algorithm starts by rasterization: creating a polygon mesh for the point cloud (e.g., via Delaunay triangulation). It then computes the centroid of each polygon in the mesh, and sorts the polygons by the depth of their centroids. Then the algorithm loops over the polygons from farthest to closest. If a near polygon covers a more distant point cloud point $p$, that point is removed.
% %works by sorting all points by their depth and looping over them from farthest to closest. If a point $p$ occurs at the same pixel $(x_{\text{cam}},y_{\text{cam}})$ as another point $p'$, but at a closer depth, then the further point $p'$ is removed. 
% This process continues until all polygons are considered. 
% The strength of this approach is that all operations inside the main loop are extremely fast. The downsides of this method are (a) the complexity of sorting large numbers of points, and (b) if polygons overlap cyclically the algorithm can fail, unless polygons are adaptively broken.


% %A downside of z-buffering is that nearer dept

% \paragraph{Ray tracing.}
% %The idea behind ray casting is
% While ray tracing is a general rendering technique that can resolve object color in 2D images, it can also be used for hidden surface determination. The simplest algorithm for ray tracing, called ray casting, works by looping through each pixel and computing the ray that begins at the viewer's eye that goes through that pixel. Different from the above methods, it does not require a rasterized polygon mesh (although it can be used with one). Another popular idea is to fit local high-order polynomials between points in order to interpolate a surface between points \cite{levin2004mesh}. However a surface is generated, the closest surface that blocks the path of the ray can be determined through an intersection test. Finally points that are surrounded by surfaces that do not intersect any ray are hidden and are removed.
% Since the late 1980s there has been extensive work on speeding up ray tracing algorithms to achieve real-time ray tracing \cite{dykstra1987brl,wald2005interactive,mcguire2019introduction}. Because of this we opt for ray tracing as our approach for identifying view-point occlusions (although in principle any of the above methods can be applied).

%(3) Mapping the points back from the camera reference frame to word reference frame. 
\paragraph{Mapping back from camera frame to world frame.}
%\subsection{Mapping Back from Camera Frame to World Frame}
%Section~\ref{Subsec:masking} described how to obtain a self-occluded 3D object that is in the camera reference frame. In these 2.5D depth image, each pixel represents an small area, whose size depend on the rendering settings, from the surfaces of the objects. On the other hand, a point t from point cloud also represents a small area of the object surface. In practice, point clouds describing the synthesized CAD models are also sampled from the mesh faces \cite{qi2017pointnet,qi2017pointnet++}.
% However, if we directly tried to learn a point cloud completion model from these camera frame point clouds, the model would have to learn additional rotational/translational invariance to identify that the occluded point clouds are actually all versions of the same original point cloud. To allow the model to focus on learning more meaningful spatial relationships, 
Once occluded points are removed, we re-project the point cloud to the original world reference frame,
% . 
%Therefore, by explicitly mapping each pixel in the depth images back from camera frame to the original world frame, we can have point clouds representing self-occluded objects. 
% This can be done with,
via the 
% following 
inverse transformation of~\eqref{eq:camera_transform}.
% \begin{align}
%       \begin{bmatrix}
%     x' \\
%     y' \\
%     z' \\
%     1  \\
%     \end{bmatrix} = 
%     \underbrace{
%     \left[
%     \begin{array}{ccc|c}
%     r_1 & r_2 & r_3 & t_1 \\
%     r_4 & r_5 & r_6 & t_2 \\
%     r_7 & r_8 & r_9 & t_3 \\
%     0   &  0  & 0   &  1
%     \end{array}
%     \right]^\top
%     }_{\big[\subalign{\;\mathbf{R}\; &| \;\mathbf{t}\; \\ \boldsymbol{0}\; &| \;1}\big]^\top}
%     \underbrace{\begin{bmatrix}
%     1/f & -\gamma/f^2 & (\gamma h - f w)/(2 f^2) & 0 \\
%     0 & 1/f      & -h/(2f) & 0 \\
%     0 & 0      & 1 & 0 \\
%     0 & 0      & 0 & 1
%     \end{bmatrix}}_{\big[\subalign{\;\mathbf{K}^{-1}\; & \;\boldsymbol{0}\; \\ \boldsymbol{0}\;\;\;\;\; & \;1}\big]}
%     \begin{bmatrix}
%         x_{\text{cam}} \\
%         y_{\text{cam}} \\
%         z_{\text{cam}} \\
%         1
%     \end{bmatrix}.
%     \label{eq:world_transform}  
% \end{align}
%Here $\mathbf{K}^{-1}$ is the inverse camera intrinsic matrix and, because rotation matrices $\mathbf{R}$ are orthogonal, we have that $\mathbf{R}^{-1} = \mathbf{R}^\top$. Thus 
% Eq.~\eqref{eq:world_transform} is the linear transformation that most closely approximates the inverse of eq.~\eqref{eq:camera_transform}, producing point $(x',y',z')$ in the world frame. 
The randomized occlusion mapping $o(\cdot)$ is constructed as follows. Fix an initial point cloud $\mathcal{P}$.
% \footnote{During implementation, we center all point clouds in the world reference frame, and apply random rotations and translations on the camera} 
% but this is equivalent, right? does it matter whether we rotate in world or camera frame? gotcha
% it is :), just one more thing, ShapeNet Occuluded is the data provided in PCN, not created by us, otherwise it won't have issues as discussed in the appendix
% the issues in appendix C? D
% can we also mention this in the appendix?
% but they didn't create this as a dataset technically did they? or... I see I see
% okay  I can change this in the experiments
% so if it's alright could you move the footnote above to the appendix and I'll fix the ShapeNet description
% cool
% Done
% they do, I use the one they realeased
% yes, just remember somewhere saying that we create ShapeNet Occuluded, which is not
% the true implementation details are, we center the objects in 
Given a camera intrinsics matrix $\mathbf{K}$, sample rotation/translation matrices $[ [\mathbf{R}_1 | \mathbf{t}_1] , \ldots, [\mathbf{R}_V | \mathbf{t}_V]]$, where $V$ is the number of views. For each view $v \in [V]$, 
%\todo{we first align the center of $\mathcal{P}$ and the center of thee camera frame},
%since eq.1 and eq.2 has implicitly assume the camera centers at the origin of the world reference frame, so we need to make it clear 
% gotcha! I will say we assume all point clouds are centered
project $\mathcal{P}$ into the camera frame of that view-point using eq.~\eqref{eq:camera_transform}, find occluded points and remove them, then map the rest back to the world reference using its inverse.
% eq.~\eqref{eq:world_transform}. 
%using z-buffering. 
% We then solve the hidden surface determination problem (e.g., via ray tracing) to remove points that are occluded in that view-point. This produces a point-cloud in the camera frame. 
%Then we map pixels whose depths are not equal to the preset buffer layer depth back to the world frame using eq.~\eqref{eq:world_transform}. 
This yields the final occluded world frame point cloud for view-point $v$: $\tilde{\mathcal{P}}_v$.

\subsection{The Completion Task}
% introduce functions encodehat we are learning in this task
Given an occluded point cloud $\tilde{\mathcal{P}}$ produced by $o(\cdot)$, the goal of the completion task is to learn a completion mapping $c: \mathbb{P} \rightarrow \mathbb{P}$ from $\tilde{\mathcal{P}}$ to a completed point cloud $\overline{\mathcal{P}}$. %Let $\tilde{\mathcal{P}} \sim o(\Pc)$ refer to a single random draw yielding an occluded point cloud. 
We say that a completion mapping is accurate w.r.t. loss $\ell(\cdot,\cdot)$ if $\mathbb{E}_{\tilde{\mathcal{P}} \sim o(\Pc)} \ell( c(\tilde{\mathcal{P}}), \Pc ) \rightarrow 0$.
The structure of the completion model $c(\cdot)$ is an ``encoder-decoder" network~\citep{3D-EPN,yuan2018pcn,Tchapmi_2019_CVPR,WangAL20}. The encoder maps an occluded point cloud to a vector, and the decoder reconstructs the full shape. After pre-training, the encoder weights can be used as initialization for downstream tasks. In appendix we gives pseudocode for OcCo and describes the architectures.




% \subsection{Point Cloud Encoder}
% Our pre-training method can work with any architecture that gives a representation $\mathbf{h}_{\mathcal{P}}$ for each point cloud $\mathcal{P}$. 
% As most modern deep learning models for point clouds output either a global point cloud representation or local pointwise representations, our method can be integrated with previous models with ease, where the local pointwise representations are aggregated using symmetric functions (e.g. max pooling) for obtaining $\mathbf{h}_{\mathcal{P}}$. 

% \subsection{Shape Completion Network}
% The shape completion network takes the representation $\mathbf{h}_{\mathcal{P}}$ of the partial point cloud as input and generates a set of points for completion. We adopt a two-stage point generation scheme following PCN \cite{yuan2018pcn}. The two-stage point scheme uses the fully-connected decoder \cite{achlioptas2017learning} to generate a sparse set of points for determining the global geometry first, then applies the folding-based decoder \cite{yang2018foldingnet} for approximating a smooth surface around the points in the sparse set.

% More specifically, a sparse set $Y_{MLP}$ of $s$ points is generated by feeding $\mathbf{h}_{\mathcal{P}}$ to a multi-layer perceptron with $3s$ output units, i.e $Y_{MLP} = \mathrm{MLP}( \mathbf{h}_{\mathcal{P}} )$. The output vector is reshaped into a matrix of size $s \times 3$, where each column represents the 3D coordinates of a point. Then, for each point $p_i$ in $Y_{MLP}$, a set $Y^i_{FOLD}$ of $u^2$ points (in a local coordinate system with $p_i$ as the origin) are generated through the folding operation \cite{yang2018foldingnet}. Every point $p_j$ of the $u^2$ points is added with $p_i$ to map it to a global coordinate system, \textit{i.e.} $p_i + p_j$. As a result, a set $Y_{FOLD}$ with $u^2 \times s$ points is obtained after taking a union of $Y^i_{FOLD}$, \textit{i.e.} $Y_{FOLD} = \cup_i Y^i_{FOLD} $. 

% \subsection{Order-Invariant Loss Functions}
% For the shape completion task, the loss function measures the differences between the generated point clouds $\mathcal{P}_1$ and ground truth point clouds $\mathcal{P}_2$. As the points in a point cloud are unordered, the loss function needs to be permutation invariant. To this end, we adopt Chamfer Distance (CD) and Earth Mover's Distance (EMD): 

% \begin{equation}
%     \mathrm{CD}(\mathcal{P}_1, \mathcal{P}_2) = \frac{1}{|\mathcal{P}_1|} \sum_{p_i \in \mathcal{P}_1} \min_{y \in \mathcal{P}_2} \Vert p_i - y \Vert_2 + \frac{1}{|\mathcal{P}_2|} \sum_{p_i \in \mathcal{P}_2} \min_{x \in \mathcal{P}_1} \Vert p_i - x \Vert_2.
%     \label{eq:cd_distance}
% \end{equation}
% CD calculates the average closest point distance between $\mathcal{P}_1$ and $\mathcal{P}_2$. The symmetric version of CD is used in Equation \ref{eq:cd_distance} to ensure that $\mathcal{P}_1$ is close to $\mathcal{P}_2$, while the points in $\mathcal{P}_2$ are covered by the points in $\mathcal{P}_1$. CD can be computed with $O(n \log n)$ complexity using efficient $k$-nearest neighbor algorithms (e.g. KDTree).

% \begin{equation}
%     \label{eq:emd_distance}
%     \mathrm{EMD}(\mathcal{P}_1, \mathcal{P}_2) = \min_{\phi: \mathcal{P}_1 \rightarrow \mathcal{P}_2} \frac{1}{|\mathcal{P}_1|} \sum_{p_i \in \mathcal{P}_1} \Vert p_i - \phi(p_i) \Vert_2.
% \end{equation}
% EMD finds a bijection function $\phi: \mathcal{P}_1 \rightarrow \mathcal{P}_2$ that minimizes the average distance between corresponding points in $\mathcal{P}_1$ and $\mathcal{P}_1$. As finding the optimal $\phi$ is computationally-expensive in practice, the iterative $(1 + \epsilon)$ approximation scheme is applied \cite{bertsekas1985distributed}. EMD with the $(1 + \epsilon)$ approximation scheme can be computed with $O(n^2)$ complexity. Empirically we have shown that both loss functions are effective in terms of performance gains of the downstream tasks.

% As we adopt the two stage generation scheme, we use the following loss function:

% \begin{equation}
%     \label{eq:loss}
%     L(Y_{MLP}, Y_{FOLD}, Y) = \mathrm{EMD}(Y_{MLP}, \hat{Y}) + \mathrm{CD}(Y_{MLP}, \hat{Y}) + \alpha \mathrm{CD}(Y_{FOLD}, Y),
% \end{equation}
% where $Y$ is the occluded set of points and $\hat{Y}$ is a sub-sampled set of points to serve as the ground truth for the sparse set $Y_{MLP}$. We did not include $\mathrm{EMD}(Y_{FOLD}, Y)$ here due to the $O(n^2)$ complexity of the earch mover's distance. $\alpha$ is a hyperparameter.


==> sections/related.tex <==
%!TEX root = ../main.tex
\qi{draw a figure summarizing previous pretrainign work. which dataset they used. it is object/scene pretraining? The fine-tuning tasks and datasets.}
% omit this, and cite a review paper
\subsection{Deep Models for Point Clouds}

Work on deep models for point clouds can largely be divided into three different structural approaches: (a) \emph{pointwise-based networks}, (b) \emph{convolution-based networks}, and (c) \emph{graph-based networks}.
We call the networks that independently process each point, before aggregating these point representations: \emph{pointwise-based networks} \citep{qi2017pointnet,qi2017pointnet++,joseph2019momen,duan2019structural,zhao2019pointweb,yang2019modeling,lin2019justlookup}. One well-known method, PointNet, devises a novel neural network that is designed to respect the permutation invariance of point clouds. Each point is independently fed into a multi-layer perceptron, then outputs are aggregated using a permutation-invariant function (e.g., max-pooling) to obtain a global point cloud representation.
% Two well-known models of this type are PointNet and PointNet++. PointNet \cite{qi2017pointnet} devises a novel neural network that is designed to respect the permutation invariance of point clouds. Each point is independently fed into a multi-layer perceptron, then outputs are aggregated using a permutation-invariant function (e.g.,  max-pooling) to obtain a global point cloud representation. However, as PointNet does not capture local structures induced by the 3D metric space, PointNet++ \cite{qi2017pointnet++} extends it by partitioning the point sets into overlapping local regions via a distance metric. It recursively groups local features into larger units to produce higher-level features. 
Another class of methods are \emph{convolution-based networks} \citep{hua2018pointwise,su2018splatnet,li2018pointcnn,atzmon2018point,landrieu2018large,hermosilla2018monte,groh2018flex,rao2019spherical}. These works map point clouds to regular grid structures and extend the classic convolution operator to handle these grid structures. 
%\paragraph{Convolution-based networks.}
%We call the networks that map point clouds to regular grid structures and extend the classic convolution operator to handle these grid structures as convolution-based networks \cite{hua2018pointwise,su2018splatnet,li2018pointcnn,atzmon2018point,landrieu2018large,hermosilla2018monte,groh2018flex,rao2019spherical}. 
A representative model, PCNN \citep{atzmon2018point}, defines two operators, extension and restriction, for mapping point cloud functions to volumetric functions and vise versa.
%To describe how models of this type function, we highlight four representative models: SPLATNet \cite{su2018splatnet}, PointCNN \cite{li2018pointcnn}, PCNN \cite{atzmon2018point} and SPG \cite{landrieu2018large}. SPLATNet \cite{su2018splatnet} maps points onto a sparse lattice, and then performs bilateral convolution only on parts of the lattice that are occupied by points. PointCNN \cite{li2018pointcnn} determines a canonical point ordering by learning a permutation and weighting of points, called an $\mathcal{X}$-transformation, before applying a conventional convolution operator. PCNN \cite{atzmon2018point} defines two operators, extension and restriction, for mapping point cloud functions to volumetric functions and vise versa. SPG \cite{landrieu2018large} focuses on dealing with large point clouds, where a superpoint graph is constructed by adaptively partitioning points into geometrically homogeneous elements. The superpoint graph is then fed into a graph neural network to produce its corresponding semantic labels. 
The third class of models is \emph{graph-based networks} \citep{simonovsky2017dynamic,wang2019dynamic,shen2018mining,wang2018local,zhang2018graph,chen2019clusternet}. These networks regard each point as a vertex of a graph and generate edges based on spatial information and node similarities. 
%as graph-based networks  \cite{simonovsky2017dynamic,wang2019dynamic,shen2018mining,wang2018local,zhang2018graph,chen2019clusternet}. 
A popular method is DGCNN \citep{wang2019dynamic}, which introduces a new operation, EdgeConv, to aggregate local features and a graph update module to learn dynamic graph relations from layer to layer. NRS~\citep{NRS} uses a neural random subspace method based on the encoded embeddings to further improve the model performance.
%PointNet++ \cite{qi2017pointnet++} also falls into this category as it assumes a fixed local graph structure during training, and uses this to compute pairwise point distances. Other graph-based point cloud models include DGCNN \cite{wang2019dynamic}, which generalizes PointNet++ by introducing a new operation, EdgeConv, to aggregate local features and a graph update module to learn dynamic graph relations from layer to layer. PointGCN \cite{zhang2018graph} combines localized graph convolutions with two types of graph downsampling operations. ClusterNet \cite{chen2019clusternet} designs a hierarchical clustering network to obtain rotation-invariant representations. 
%\newline

%\noindent
%we propose a new pre-training method that can be used for any of the above existing architectures to accelerate training.
%that is applicable to existing architectures.
% HERERE

\subsection{Pre-Training for Point Clouds}
Pre-training models on unlabelled data are gaining popularity recently due to its success on a wide range of tasks, such as natural language understanding \citep{mikolov2013efficient,devlin2018bert}, object detection \citep{he2019momentum,chen2020simple} and graph representations \citep{hu2019pre,GPT}. 
The representations learned from these pre-trained models can be used as a good initializer in downstream tasks, where task-specific annotated samples are scarce. 
The three most common pre-training objectives for point clouds are based on:
(i) generative adversarial networks (GAN), (ii) autoencoders, and (iii) spatial relation. 
However, GANs for point clouds are limited to non-point-set inputs, i.e., voxelized representations~\citep{wu2016learning}, 2D depth images of point clouds \citep{han2019view}, and latent representations from autoencoders \citep{achlioptas2017learning}, as sampling point sets from a neural network is non-trivial. Thus these GAN approaches cannot leverage the natural order-invariance of point-sets. 
Autoencoders \citep{yang2018foldingnet,li2018so,hassani2019unsupervised,ShiXYF20} learn to encode point clouds into a latent space before reconstructing these point clouds from their latent representation. 
Similar to these methods, generative models based on normalizing flow~\citep{pointflow} and approximate convex decomposition~\citep{gadelha2020label} have been shown effective for the unsupervised learning on point clouds. 
% \todo{Yet, there is recent evidence that the representations learned by autoencoders are not necessarily good when used as initialization for downstream tasks~\citep{alberti2017pitfall}.}
However, both GAN and autoencoder-based pre-training methods have been recently outperformed on downstream tasks by the pre-training technique of~\citet{sauder2019self} or~\citet{sharma2020self} in few-shot setting.
%and \citet{alliegro2020joint}.

These methods are based on spatial relation reconstruction, %which can be seen as an extension of solving jiggle puzzles in 2D images \cite{NorooziF16}. 
which aims to reconstruct points clouds given rearranged point clouds as input. To this end, \citet{sauder2019self} equally split the 3D space into $k^3$ voxels, rearrange $k^3$ voxels and train a model to predict the original voxel label for each point. However, these random permutations destroy all spatial information that the model could have used to predict the true point cloud. 
Inspired by cover-trees~\citep{beygelzimer2006cover}, \citet{sharma2020self} utilised ball covers for hierarchical partitioning of points. They then train a model to classify each point to their assigned clusters. However, the selection of the ball centroids is somewhat random and they need to pre-train from scratch for each fine-tuning task. 
% \citep{alliegro2020joint} further developed this approach into % 3D puzzle solving task into a multi-task learning framework where other tasks are supervised, i.e. classification and part segmentation.
Instead, our method creates spatially realistic occlusions that a completion model learns to reconstruct. As such, this model learns how to naturally encode 3D object shape and contextual information. Recently there is a new method called PointContrast~\citep{pointcontrast} which mainly uses contrastive learning for pre-training indoor segmentation models. Our method is more general and transferable compared with theirs. 

Point cloud completion~\citep{yuan2018pcn} has received attentions in recent years. Most works aim at achieving a lower reconstruction loss by incorporating 1) a better encoder~\citep{xie2020grnet,huang2020pf}, 2) a better decoder~\citep{Tchapmi_2019_CVPR,wen2020point}; 3) cascaded refinement~\citep{WangAL20} and 4) multi-viewed consistency~\citep{hu20203d}.

Completing 3D shapes for model initialisation has been considered before. \citet{schonberger2018semantic} used scene completion~\citep{song2017semantic,dai2020sg,hou2020revealnet} as an auxiliary task to initialise 3D voxel descriptors for visual localisation. 
They generated nearly-complete and partial voxelised scenes based on depth images and trained a variational autoencoder for completion. They have showed that the pre-trained encoder is more robust under different viewpoints and weather conditions. %However, they do not explicitly show that the pre-training brings improvements since the lack of the control group (i.e., training from scratch.)
% SG-NN~\citep{dai2020sg} and RevealNet~\citep{hou2020revealnet} specifically tackles the unsupervised scene completion task  by inferring unobserved scene geometry. 
We adapt this idea to pre-training for point clouds. We have shown that our initialisation is better than random and prior methods in terms of 1) object understanding; 2) invariance under transformations; and 3) downstream task performance.
% based we show that such learned embeddings are also robust to transformation and 
% \todo{Compared to these works OcCo is different in a significant way: our approach only learn pre-trained weights on a single dataset (ModelNet40). We have shown that such pre-trained weights outperform all point cloud baselines in few-shot learning, improve generalization on many different classification tasks, and have better transformation invariance than prior work. As far as we are aware it was not known that such pre-training would yield such improvements across tasks and datasets.}
% Compared with these works, 
% in \abbrev, 
% On this basis, 
% we have provided more in-depth and interpretable analysis on the learned representations after pre-training as well as shown more transferable ability. 

%On the basis of these, we provide more in-depth analysis of the pre-training process with network dissection and invariance under SO(3) transformation. We further show that completing the occluded objects~\citep{yuan2018pcn,Tchapmi_2019_CVPR,WangAL20,WenLHL20} is transferable to improve the generalisation of various downstream tasks as well as label efficiency.
% However, our method show that the 3D completion task 
%Instead we propose a method utilizing the occlusion completion, where the objective directly takes point clouds as input and completes the partial point clouds based on spatial relations. Compared with Sauder and Sievers \cite{sauder2019self} and Alliegro et al.\cite{alliegro2020joint}, our method purely origins from the 3D vision perspective and achieves better results with the same baselines on both synthetic and real-world datasets. 
%In this paper, our goal is to propose a novel pre-training mechanism that can be used to learn initialization for any of the above architectures. These initialization will accelerate training and improve generalization.
%Before we describe our method, we review current work in pre-training methods for point clouds, their shortcomings, and how our approach will address these.

% \subsection{Pre-training for Images}
% Pre-training~(a.k.a. self-supervised learning) has been widely used on images. Inspired by the unsupervised method~\cite{mikolov2013efficient} from natural language processing domain which rely on predicting works from their context, ~\cite{doersch2015relative} proposed a practically successful pre-training task of predicting the relative location of image patches. After this work,~\cite{noroozi2016jigsaw} introduced a method predicting the permutation of a ``jigsaw puzzle'' which is created from the full images. In contrast to these patch-based methods, some methods generate cleverly designed image-level classification tasks. In~\cite{gidaris2018rotation}, an image is randomly rotated by one of four possible angles and let the model predict the rotation. Another class of pre-training tasks contains tasks with dense spatial outputs. Some examples are image colorization~\cite{zhang2016colorful}, split-brain autoencoders~\cite{zhang2017split}, image inpainting~\cite{pathak2016context}, and motion segmentation prediction~\cite{pathak2017learning}. 


==> sections/related_new.tex <==
%!TEX root = ../main.tex

% omit this, and cite a review paper
% The current developments in deep point cloud models can be referred to~\cite{9127813}.

Pre-training models on unlabelled data are gaining popularity recently due to its success on a wide range of tasks, such as natural language understanding \citep{mikolov2013efficient,devlin2018bert}, object detection \citep{he2019momentum,chen2020simple} and graph representations \citep{hu2019pre,GPT}. 
The representations learned from these pre-trained models can be used as a good initializer in downstream tasks, where task-specific annotated samples are scarce. 
The three most common pre-training objectives for point clouds are based on:
(i) generative adversarial networks (GAN), (ii) autoencoders, and (iii) spatial relation. 
However, GANs for point clouds are limited to non-point-set inputs, i.e., voxelized representations~\citep{wu2016learning}, 2D depth images of point clouds \citep{han2019view}, and latent representations from autoencoders \citep{achlioptas2017learning}, as sampling point sets from a neural network is non-trivial. Thus these GAN approaches cannot leverage the natural order-invariance of point-sets. 
Autoencoders \citep{yang2018foldingnet,li2018so,hassani2019unsupervised,ShiXYF20} learn to encode point clouds into a latent space before reconstructing these point clouds from their latent representation. 
Similar to these methods, generative models based on normalizing flow~\citep{pointflow} and approximate convex decomposition~\citep{gadelha2020label} have been shown effective for the unsupervised learning on point clouds. 
% \todo{Yet, there is recent evidence that the representations learned by autoencoders are not necessarily good when used as initialization for downstream tasks~\citep{alberti2017pitfall}.}
However, both GAN and autoencoder-based pre-training methods have been recently outperformed on downstream tasks by the pre-training technique of~\citet{sauder2019self} or~\citet{sharma2020self} in few-shot setting.
%and \citet{alliegro2020joint}.

These methods are based on spatial relation reconstruction, %which can be seen as an extension of solving jiggle puzzles in 2D images \cite{NorooziF16}. 
which aims to reconstruct points clouds given rearranged point clouds as input. To this end, \citet{sauder2019self} equally split the 3D space into $k^3$ voxels, rearrange $k^3$ voxels and train a model to predict the original voxel label for each point. However, these random permutations destroy all spatial information that the model could have used to predict the true point cloud. 
Inspired by cover-trees~\citep{beygelzimer2006cover}, \citet{sharma2020self} utilised ball covers for hierarchical partitioning of points. They then train a model to classify each point to their assigned clusters. However, the selection of the ball centroids is somewhat random and they need to pre-train from scratch for each fine-tuning task. 
Instead, our method creates spatially realistic occlusions that a completion model learns to reconstruct. As such, this model learns how to naturally encode 3D object shape and contextual information. Recently there is a new method called PointContrast~\citep{pointcontrast} which mainly uses contrastive learning for pre-training indoor segmentation models. \todo{add a few on contrastive works}
% Our method is more general and transferable compared with theirs. 

% Point cloud completion~\citep{yuan2018pcn} has received attentions in recent years. Most works aim at achieving a lower reconstruction loss by incorporating 1) a better encoder~\citep{xie2020grnet,huang2020pf}, 2) a better decoder~\citep{Tchapmi_2019_CVPR,wen2020point}; 3) cascaded refinement~\citep{WangAL20} and 4) multi-viewed consistency~\citep{hu20203d}.

Completing 3D shapes for model initialisation has been considered before. \citet{schonberger2018semantic} used scene completion~\citep{song2017semantic,dai2020sg,hou2020revealnet} as an auxiliary task to initialise 3D voxel descriptors for visual localisation. 
They generated nearly-complete and partial voxelised scenes based on depth images and trained a variational autoencoder for completion. They have showed that the pre-trained encoder is more robust under different viewpoints and weather conditions. %However, they do not explicitly show that the pre-training brings improvements since the lack of the control group (i.e., training from scratch.)
% SG-NN~\citep{dai2020sg} and RevealNet~\citep{hou2020revealnet} specifically tackles the unsupervised scene completion task  by inferring unobserved scene geometry. 
We adapt this idea to pre-training for point clouds. We have shown that our initialisation is better than random and prior methods in terms of 1) object understanding; 2) invariance under transformations; and 3) downstream task performance.

